When is Agnostic Reinforcement Learning Statistically Tractable?

We study the problem of agnostic PAC reinforcement learning (RL): given a policy class $\Pi$, how many rounds of interaction with an unknown MDP (with a potentially large state and action space) are required to learn an $\epsilon$-suboptimal policy with respect to $\Pi$? Towards that end, we introduce a new complexity measure, called the \emph{spanning capacity}, that depends solely on the set $\Pi$ and is independent of the MDP dynamics. With a generative model, we show that for any policy class $\Pi$, bounded spanning capacity characterizes PAC learnability. However, for online RL, the situation is more subtle. We show there exists a policy class $\Pi$ with a bounded spanning capacity that requires a superpolynomial number of samples to learn. This reveals a surprising separation for agnostic learnability between generative access and online access models (as well as between deterministic/stochastic MDPs under online access). On the positive side, we identify an additional \emph{sunflower} structure, which in conjunction with bounded spanning capacity enables statistically efficient online RL via a new algorithm called POPLER, which takes inspiration from classical importance sampling methods as well as techniques for reachable-state identification and policy evaluation in reward-free exploration.

==> sections/app_lower_bound_proof.tex <==
\section{Proof of \pref{thm:lower-bound-online}} 

==> sections/lower-bound.tex <==
\newpage
\section{Lower Bound}\label{sec:lower-bound}

We prove a superpolynomial lower bound on the sample complexity required to learn bounded \dimname{} classes.

\begin{theorem}[Lower bound for bounded \dimname{}]\label{thm:lower-bound-online}
\gene{A placeholder for now until we have a more concrete statement.}
Let $\eps \in (0,1)$, $H \ge \dots$, $\ell \in [H]$. There exists a policy class $\Piell$ of size $O(1/\eps^\ell)$ with $\dimRL(\Piell) \le O(H^{4\ell+2})$ and a family of MDPs $\cM$ with state space $\cS$ satisfying $\abs{\cS} = H\cdot 2^{H+1}$, binary action space, horizon $H$ such that: any algorithm $\alg$ that returns an $\eps$-optimal policy with probability at least $1/4$, there exists an $M \in \cM$ on which $\alg$ collects at least 
\begin{align*}
    \Omega\Big(\min \big\{\frac{1}{\eps^\ell}, 2^{H/2} \big\} \Big) \quad \text{trajectories}. 
\end{align*}
\end{theorem}

Some remarks
\begin{itemize}
    \item State space satisfies $\log \abs{\cS} \le O(H)$.
    \item Policy class is realizable, i.e. $\pistar \in \Piell$, and small since $\log \abs{\Piell} \le \ell \log(1/\eps)$.
    \item Thus this rules out $\poly(H, \dimRL(\Pi), \log \abs{\Pi}, \log \abs{\cS}, 1/\eps)$ upper bound in general. We must have at least $1/\eps^{\log \dimRL(\Pi)}$ dependence.
\end{itemize}

\subsection{Boolean Matrix Construction} 
First we define a block-free property of boolean matrices.
\begin{definition}\label{def:intersection-property}
Fix parameters $k, \ell \in \bbN$. We say a binary matrix $B \in \crl{0,1}^{N \times d}$ is \textbf{$(k, \ell)$ block-free} if the following holds: for every $I \subset [N]$ with $\abs{I} = k$, and $J \subset [d]$ with $\abs{J} = \ell$ there exists some $(i,j)\in I\times J$ with $B_{ij} = 0$.
\end{definition}

In words, matrices which are $(k,\ell)$ block-free do not contain a $k\times \ell$ ``block'' of all 1s.

\begin{lemma}\label{lem:matrix-construction}
Fix any $\eps \in (0,1/10)$ and $\ell \in \bbN$. For any 
\begin{align*}
    d \in \Big[ \frac{16 \ell \cdot \log(1/\eps)}{\eps}, \frac{1}{20} \cdot \exp\Big( \frac{1}{48 \cdot \eps^{\ell-1}} \Big) \Big] ,
\end{align*}
there exists a boolean matrix $B \in \crl{0,1}^{N\times d}$ with $N = 1/(6 \cdot \eps^\ell)$ such that:
\begin{enumerate}
    \item (Row sum): for every row $i \in [N]$, we have $\sum_{j} B_{ij} \ge \eps d /2$.
    \item (Column sum): for every column $j \in [d]$, we have $\sum_{i} B_{ij} \in [\eps N /2, 2\eps N]$.
    \item The matrix $B$ is $(\ell \log d,\ell)$ block-free.
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of \pref{lem:matrix-construction}.]
The existence of $B$ is proven by a probabilistic argument. Let $\wt{B} \in \crl{0,1}^{N\times d}$ be a random matrix where each entry is i.i.d. chosen to be 1 with probability $\eps$.

By Chernoff bounds, for every row $i \in [N]$, we have $\P\brk{\sum_{j} B_{ij} \le \tfrac{\eps d}{2}} \le \exp\prn{-\eps d /8}$; likewise for every column $j \in [d]$ we have $\P\brk{\sum_{j} B_{ij} \notin \brk{\tfrac{\eps N}{2}, 2\eps N}} \le 2\exp\prn{-\eps N /8}$. By union bound, the matrix $\wt{B}$ satisfies the first two properties with probability at least $0.8$ as long as 
\begin{align*}
    d \ge (8 \log 10N)/\eps, \quad \text{and} \quad N \ge (8 \log 20d)/\eps.
\end{align*}
One can check that under the choice of $N = 1/(6 \cdot \eps^\ell)$, both constraints are met.

Now we examine the probability of $\wt{B}$ satisfies the block-free property with parameters $(k = \ell \log d, \ell)$. Let $X$ be the random variable which denotes the number of violations to the block-free property in $\wt{B}$, i.e., 
\begin{align*}
    X = \abs{ \crl{I \times J: I \subset [N], \abs{I} = k, J \subset [d], \abs{J} = \ell, \wt{B}_{ij} = 1 \ \forall \ (i,j)\in I \times J} }. 
\end{align*}
By linearity of expectation we have
\begin{align*}
    \bbE \brk{X} \le N^{k} d^\ell \eps^{k \ell}.
\end{align*}
We now plug in the choice $k = \ell \log d$ and observe that as long as $N \le 1/(2e \cdot \eps^\ell)$ we have $\bbE[X] \le 1/2$. By Markov's inequality, $\P[X = 0] \ge 1/2$.

Therefore with positive probability, $\wt{B}$ satisfies all 3 properties (otherwise we would have a contradiction via inclusion-exlusion principle). We can conclude the existence of $B$ which satisfies all 3 properties, proving the result.
\end{proof}

\subsection{Construction of state space, action space, and policy class}
\paragraph{State and action spaces.}
First we define the state space $\cS$. In every level $h \in [H]$, there will be $2^{H+1}$ states. The states will be paired up, and each state will be represented by either $\jof{h}$ or $\jpof{h}$, so $\cS_h = \crl{\jof{h}: j \in [2^H]} \cup \crl{\jpof{h}: j \in [2^H]}$. For any state $s \in \cS$, we define the \emph{index} of $s$, denoted $\idx(s)$ as the unique $j\in [2^H]$ such that $s \in \crl{\jof{h}}_{h\in[H]} \cup \crl{\jpof{h}}_{h\in[H]}$. In total there are $H \cdot 2^{H+1}$ states. The action space is $\cA = \crl{0,1}$.

\paragraph{Policy class.} For the given $\eps$ and $\ell \in \crl{1, 2, \dots, H}$ we will use \pref{lem:matrix-construction} to construct a policy class $\Piell$ which has bounded \dimname{} but is hard to explore. We instantiate \pref{lem:matrix-construction} with $\ell$ and $d = 2^H$, and use the resulting matrix $B$ to construct $\Piell = \crl{\pi_i}_{i\in [N]}$ with $\abs{\Piell} = N = O(1/\eps^\ell)$. We will consider the setting when $2\eps N < 2^H$ (this is mild, and is satisfied whenever $\eps = 1/\poly(H)$). We define the policies as follows: for every $\pi_i \in \Piell$ we set
\begin{align*}
    \text{for every } j \in [2^H]: \quad&\pi_i(\jof{h}) = \pi_i(\jpof{h}) = \begin{cases}
    \bit_h(\sum_{a \le i} B_{aj}) &\text{if} \ B_{ij} =1,\\
    0 & \text{if} \ B_{ij} = 0.
    \end{cases} \numberthis\label{eq:pi-construction}
\end{align*}
The function $\bit_h: [2^H-1] \to \crl{0,1}$ selects the $h$-th bit in the binary representation of the input.

Now we list several properties that $\Piell$ satisfies, which will be useful for proof of the lower bound. We introduce the notation for any $j \in [2^H]$ to denote $\Piell_j := \crl{\pi \in \Piell: \exists h \in [H], \pi(\jof{h}) = 1}$.  We also use for any $\pi \in \Piell$ the notation  $\Srel^\pi := \crl{j \in [2^H]: \pi \in \Piell_j}$ to denote the relevant states for a given policy. \gene{Eventually I think we can just move the boolean matrix construction to the appendix and only have a lemma in main text which states existence of some policy class which satisfies these properties.}

\begin{lemma}\label{lem:piell-properties}
The policy class $\Piell$ satisfies the following properties. 
\begin{itemize}
    \item[(1)] For every $j \in [2^H]$ we have $\abs{\Piell_j} \in  [\eps N/2, 2\eps N]$.
    \item[(2)] For every $\pi \in \Pi$ we have $\abs{ \Srel^\pi } \ge \eps/2 \cdot 2^H$.
    \item[(3)] For every $\pi \in \Piell_j$, the vector $(\pi(\jof{1}), \dots, \pi(\jof{H})) \in \crl{0,1}^H$ is unique.
    \item[(4)] Bounded \dimname{}: $\dimRL(\Piell) \le c \cdot H^{4\ell+2}$ for some absolute numerical constant $c > 0$.\gene{I am using the $\max_h$ version of the definition.}
\end{itemize}
\end{lemma}

\begin{proof}[Proof of \pref{lem:piell-properties}.]
Properties (1)-(3) are straightforward from the construction of $B$ and $\Piell$, since $\pi_i \in \Piell_j$ if and only if $B_{ij} = 1$. We require that $2\eps N < 2^H$ in order for Property (3) to hold.

We now prove Property (4): that $\Piell$ has bounded \dimname{}. To prove this we will use the block-free property of the underlying boolean matrix $B$.

Fix any deterministic MDP $M$ which witnesses $\dimRL(\Piell)$. To bound $\dimRL(\Piell)$, we need to count the contribution to $\dimRL(\Piell)$ from distinct trajectories $\tau$ which are produced by some $\pi \in \Piell$ on $M$. We first define a \emph{level decomposition} for a trajectory $\tau = (s_1, a_1, s_2, a_2, \dots, s_H, a_H)$. We define the level decomposition'' of $\tau$ as the unique tuple of indices $(h_1, h_2, \dots h_{m})$, where each $h_k \in [H]$. The level decomposition satisfies the following properties:
\begin{itemize}
    \item The levels satisfy $h_1 < h_2 < \dots < h_m$.
    \item The level $h_1$ represents the first level where $a_{h_1} = 1$.
    \item The level $h_2$ represents the first level where $a_{h_2} = 1$ on some state $s_{h_2}$ such that
    \begin{align*}
        \idx(s_{h_2}) \notin \crl{ \idx(s_{h_1}) }.
    \end{align*}
    \item The level $h_3$ represents the first level where $a_{h_3} = 1$ on some state $s_{h_3}$ such that 
    \begin{align*}
        \idx(s_{h_3}) \notin \crl{ \idx(s_{h_1}), \idx(s_{h_2}) }.
    \end{align*}
    \item More generally the level $h_k$, $k\in[m]$ represents the first level where $a_{h_k} = 1$ on some state $s_{h_k}$ such that 
    \begin{align*}
         \idx(s_{h_k}) \notin \crl{ \idx(s_{h_1}), \dots, \idx(s_{h_{k-1}}) }.
    \end{align*}
    In other words, the level $h_k$ represents the hitting level of action $a=1$ on a new state index which $\tau$ has never played $a=1$ on before.
\end{itemize} 

We will count the contribution to $\dimRL(\Piell)$ by doing casework on the length of the level decomposition. Since the level decomposition of a trajectory is unique, the sets of trajectories with $m$-length level decompositions are unique. We will use the shorthand $\jexp{k} := \idx(s_{h_k})$ for all $k\in [m]$.
\begin{itemize}
    \item (Case: $m=0$) The trajectory $\tau$ must take 0 at all times. There is one such $\tau$, so the contribution towards $\dimRL(\Piell)$ here is 1.
    \item (Case: $m=1$) We have $H$ choices for $(h_1)$; once we have committed to some $h_1 \in [H]$ we have committed to only playing $a=1$ on state index $j^{(1)}$. Thus the contribution for each choice of $h_1$ is at most $2H$. In total, the contribution for trajectories which satisfy $m=1$ to $\dimRL(\Piell)$ is at most $2H^2 = O(H^2)$. \gene{this is done using the layerwise argument, but I have omitted the details right now.}
    \item (Case: $m=2$)  We have at most $H^2$ choices for the tuple $(h_1, h_2)$. For any fixed tuple $(h_1, h_2)$ there is a unique choice for $j^{(1)}$, and then there are $2H$ possibilities for $j^{(2)}$. Once we have fixed $j^{(1)}$ and $j^{(2)}$ we are restricted to playing 1 on those two state indices henceforth, and the contribution to $\dimRL(\Piell)$ is at most $4H$ afterwards. Thus the total contribution is $H^2 \times (2H) \times (4H) = O(H^4)$.
    \item We can continue in this fashion and show that for every $m \le \ell$ we have the contribution is at most 
    \begin{align*}
        H^m \times \prod_{k=1}^m (2kH) = O(H^{4m}).
    \end{align*}
    \item What happens for $m > \ell$? Observe that the block-free property on $B$ implies that for any $J \subseteq [2^H]$ with $\abs{J} = \ell$ we have $\abs{\cap_{j \in J} \Pi_j} \le \ell \log 2^H = O(\ell H)$. So for any trajectory $\tau$ with level decomposition such that $m > \ell$ we know that there is at most $O(\ell H)$ contribution to the $\dimRL(\Piell)$ after we have taken the $\ell$-th 1 action at level $h_{\ell}$. Therefore for these such trajectories, their contribution to $\dimRL(\Piell)$ is at most $O(\ell \cdot H^{4\ell+1})$.
\end{itemize}
Therefore, summing over all the cases, we have the bound that
\begin{align*}
    \dimRL(\Piell) \le \Big(\sum_{m \le \ell} O(H^{4m})\Big) + O(\ell \cdot H^{4\ell+1}) \le O(H^{4\ell+2}).
\end{align*}
This concludes the proof of the lemma.
\end{proof}

\subsection{Construction of MDP family}
The family $\cM = \crl{M_{\pistar,\phi}}_{\pistar \in \Piell, \phi \in \Phi}$ will be a family of MDPs which are indexed by a policy $\pistar$ as well as a \emph{decoder} function $\phi: \cS \to \crl{\mathsf{good}, \mathsf{bad}}$, which assigns each state to be ``good'' or ``bad'' in a sense that will be described later on.

\paragraph{Decoder function class.} The decoder function class $\Phi$ will be all possible mappings which for every $j\in [2^H]$, $h \ge 2$ assign exactly one of $\jof{h}, \jpof{h}$ to the label $\mathsf{good}$ and the other one to $\mathsf{bad}$. There are $(2^{H-1})^{2^H}$ such functions. The label of a state will be used to describe the transition dynamics. Intuitively, a learner who does not know the decoder function $\phi$ will not be able to tell if a certain state has the label  $\mathsf{good}$ or $\mathsf{bad}$ upon visiting a state index $j$ for the first time.

\paragraph{Transition dynamics.} The MDP $M_{\pistar, \phi}$ will be a uniform distribution over $2^H$ combination locks $\crl{\mathsf{CL}_j}_{j \in [2^H]}$ with disjoint states. More formally, $s_1 \sim \mathsf{Unif}(\{\jof{1}\}_{j\in[2^H]})$. From each start state $\jof{1}$, only the $2H-2$ states corresponding to index $j$ at levels $h>1$ will be reachable in combination lock $\mathsf{CL}_j$.

Now we will describe each combination lock $\mathsf{CL}_j$, which forms the basic building block of the MDP construction.

\begin{itemize}
    \item \textbf{Good/bad set.} At every level $h\in [H]$, for each $\jof{h}$ and $\jpof{h}$, the decoder function $\phi$ assigns one of them to be $\mathsf{good}$ and one of them to be $\mathsf{bad}$. We will henceforth denote $\jgof{h}$ to be the good state and $\jbof{h}$ to be the bad state. Observe that by construction in Eq.~\pref{eq:pi-construction}, for every $\pi \in \Piell$ and $h\in [H]$ we have $\pi(\jgof{h}) = \pi(\jbof{h})$.
    \item \textbf{Dynamics of $\mathsf{CL}_j$, if $j\in \Srel^\pistar$.} Here, the transition dynamics of the combination locks are deterministic. We let $T(s,a)$ denote the state that $(s,a)$ transitions to, i.e., $T(s,a) = s'$ if and only if $P(s'|s,a) = 1$. We also use $T(s,\pi) := T(s, \pi(s))$ as shorthand. For every $h\in [H]$,
    \begin{itemize}
        \item On good states $\jgof{h}$ we transit to the next good state iff the action is $\pistar$: \begin{align*}
            T(\jgof{h}, \pistar) = \jgof{h+1}, \quad \text{and} \quad T(\jgof{h}, 1-\pistar) = \jbof{h+1}.
        \end{align*}
        \item On bad states $\jbof{h}$ we always transit to the next bad state: 
        \begin{align*}
            T(\jbof{h}, a) = \jbof{h+1}, \quad \text{for all } a \in \cA.
        \end{align*}
    \end{itemize}
    \item \textbf{Dynamics of $\mathsf{CL}_j$, if $j\notin \Srel^\pistar$.} If $j$ is not a relevant state for $\pistar$, then the transitions are random regardless of the current state/action:
    \begin{align*}
    \text{for all $j$ and $h\in[H]$}, \quad T(\jgof{h},a) = T(\jbof{h}, a) = \mathrm{Unif}(\crl{\jgof{h+1}, \jbof{h+1}}.
\end{align*}
    \item \textbf{Reward structure.} The reward function is nonzero at level $H$, and is defined as 
    \begin{align*}
        R(s_H,a) = \mathrm{Ber}\prn*{ \frac{1}{2} + \frac{1}{4} \cdot \mathbbm{1}\crl{\pistar \in \Piell_j} \cdot \mathbbm{1}\crl{s_H = \jgof{H}, a = \pistar(\jgof{H})} }
    \end{align*}
    That is, we get $3/4$ whenever we reach the $H$-th good state for a state index $j$ which is relevant for $\pistar$, and $1/2$ reward otherwise.
\end{itemize}

\paragraph{Reference MDP $M_0$.} We define a \emph{reference MDP} $M_{0}$. In the reference MDP $M_0$, all the combination locks behave the same and have uniform transitions to the next state. The distribution over all $2^H$ combinations is again taken to be the uniform distribution. The rewards for $M_0$ will be $\mathrm{Ber}(1/2)$ for every $(s,a) \in \cS_H\times \cA$.

\subsection{Proof of \pref{thm:lower-bound-online}}
Now we are ready to prove the lower bound using the construction $\cM$.

\paragraph{Value calculation.} Consider any $M_{\pistar,\phi} \in \cM$. For any policy $\pi \in \cA^{\cS \times[H]}$ we use $V_{\pistar,\phi}(\pi)$ to denote the value of running $\pi$ in MDP $M_{\pistar,\phi}$. By construction we can see that
\begin{align*}
    V_{\pistar,\phi}(\pi) = \frac{1}{2} + \frac{1}{4} \cdot \Pr_{\pistar,\phi}\brk*{ s_1 \in \Srel^\pistar \wedge \pi(s_{1:H}) = \pistar(s_{1:H}) }.\numberthis\label{eq:value-of-pi}
\end{align*}
Here we use $\pi(s_{1:H}) \in \crl{0,1}^H$ to denote the sequence of actions that $\pi$ takes on the $H$ states $\jof{1}, \dots, \jof{H}$ where $j = \idx(s_1)$. In other words, the expectation captures the probability (over the initial starting state) that $\pi$ solves a combination lock rooted at a relevant state $s_1 \in \Srel^\pistar$. By Property (2) and (3) of \pref{lem:piell-properties}, we additionally have that $V_{\pistar,\phi}(\pistar) \in \brk{ 1/2 + \eps/8, 1/2 + \eps/2 }$.

By Eq.~\pref{eq:value-of-pi}, if $\pi$ is an $\eps/16$-optimal policy on $M_{\pistar,\phi}$ it must satisfy
\begin{align*}
    \Pr_{\pistar,\phi}\brk*{ s_1 \in \Srel^\pistar \wedge \pi(s_{1:H}) = \pistar(s_{1:H}) } \ge \frac{\eps}{4}.
\end{align*}

\paragraph{Averaged measures.} We define the following measures which will be used in the analysis. First, let us define $\Pr_\pistar[\cdot] = \frac{1}{\abs{\Phi}} \sum_{\phi \in \Phi} \Pr_{\pistar, \phi}[\cdot]$ to be the averaged measure where we first pick $\phi$ uniformly among all decoders and then consider the distribution induced by $M_{\pistar, \phi}$. Also, let the MDP $M_{0, \pistar, \phi}$ have the same transitions as $M_{\pistar, \phi}$ but with rewards at the last layer to be $\mathrm{Ber}(1/2)$, the same as the rewards for $M_0$. Then we can define the averaged measure $\Pr_{0, \pistar}[\cdot] = \frac{1}{\abs{\Phi}} \sum_{\phi \in \Phi} \Pr_{0, \pistar, \phi}[\cdot]$ where we pick $\phi$ uniformly and then consider the distribution induced by $M_{0, \pistar, \phi}$. For both averaged measures the expectations $\En_{\pistar}$ and $\En_{0, \pistar}$ are defined analogously.

\paragraph{Algorithm and stopping time.}
Recall that learning rule $\alg$ is comprised of two phases. In the first phase, it collects some number of trajectories by interacting with the MDP in episodes. We use $\st$ to denote the (random) number of episodes after which $\alg$ terminates. We also use $\alg_t$ to denote the intermediate policy that the algorithm runs in round $t$ for $t \le \st$. In the second phase, $\alg$ outputs a policy $\pihat$. We use the notation $\algout: \crl{\tau^t}_{t \in [\st]} \to \cA^{\cS\times [H]}$ to denote the second phase of $\alg$ which outputs the $\pihat$ as a measurable function of collected data.

For any policy $\pistar$, decoder $\phi$, and dataset $\cD$ we define the event
\begin{align*}
    \cE(\pistar, \phi, \cA(\cD)) := \ind{ \Pr_{\pistar,\phi}\brk*{ s_1 \in \Srel^\pistar~ \text{and}~ \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } \ge \frac{\eps}{4} }
\end{align*}
The randomness in $\cE(\pistar, \phi, \cA(\cD))$ is due to randomness in $\cD$, the data collection process of $\alg$ (which includes the underlying MDP on which $\alg$ is run). Note that the event $\cE$ is well defined for $\cD$ that is collected on \emph{any} MDP, not just $M_{\pistar,\phi}$.

Under this notation, the PAC learning guarantee on $\alg$ implies that for every $\pistar \in \Piell$, $\phi \in \Phi$ we have
\begin{align*}
    \En_{\pistar,\phi} \brk*{ \cE(\pistar, \phi, \cA(\cD)) } \ge 1-\delta. \numberthis \label{eq:pac-guarantee-exp-per-decoder} 
\end{align*}
Moreover we also have
\begin{align*}
    \En_{\pistar} \brk*{ \cE(\pistar, \phi, \cA(\cD)) } \ge 1-\delta. \numberthis \label{eq:pac-guarantee-exp} 
\end{align*}

For the lower bound argument, we apply a truncation to the stopping time $\st$. Denote \gene{not sure yet}
\begin{align*}
    \Tmax := \frac{1}{\delta} \cdot \dots
\end{align*}
Observe that if $\Pr_\pistar \brk{\st > \Tmax} > \delta$ for some $\pistar \in \Piell$ then the lower bound immediately follows, since
\begin{align*}
    \max_{\phi \in \Phi} \En_{\pistar, \phi}[\st] > \En_{\pistar}[\st] \ge \Pr_{\pistar}[\st > \Tmax] \cdot \Tmax \ge \delta \Tmax,
\end{align*}
so there must exist an MDP $M_{\pistar, \phi}$ for which $\alg$ collects at least $\delta\Tmax$ samples in expectation.

Otherwise we have $\Pr_\pistar \brk{\st > \Tmax} \le \delta$ for all $\pistar \in \Piell$. This further implies that for all $\pistar \in \Piell$
\begin{align*}
    \Pr_\pistar \brk*{\st < \Tmax \wedge \cE(\pistar, \phi, \cA(\cD))} \ge 1-2\delta.
\end{align*}
In this second case, we will show that $\alg$ requires a lot of samples on $M_0$. This is formalized in the following lemma.
\begin{lemma}[Stopping time lemma]\label{lem:stopping-time}
Let $\alg$ be an $(\eps/16,\delta)$-PAC  algorithm. Let $\Tmax \in \bbN$.  Suppose that $\Pr_\pistar \brk*{\st < \Tmax \wedge \cE(\pistar, \phi, \cA(\cD))} \ge 1-2\delta$ for all $\pistar \in \Piell$. The expected stopping time for $\alg$ on $M_0$ is at least
\begin{align*}
    \En_0 \brk*{\st} \ge \prn*{ \abs{\Piell} - \frac{4}{\eps}} \cdot \log \prn*{\frac{1}{ 2 \delta }} - \abs{\Piell} \log(2) - \abs{\Piell} \Tmax \Delta(\Tmax) \log \prn*{\frac{e}{ 2 \delta }}.
\end{align*}
\end{lemma}

The function $\Delta(\Tmax)$ is defined in \pref{lem:change_measure} to be $\dots$, so plugging in this in we see that 
\begin{align*}
    \En_0[\st] \ge \dots.
\end{align*}
This concludes the proof of \pref{thm:lower-bound-online}.\qed

\subsection{Proof of \pref{lem:stopping-time}}

For any $\pistar \in \Piell$ we denote the random variable
\begin{align*}
N^\pistar = \sum_{t=1}^{\st \wedge \Tmax} \ind{\alg_t(s_{1:H}) = \pistar(s_{1:H}) \wedge s_1 \in \Srel^\pistar},
\end{align*}
the number of episodes for which the algorithm's policy matches that of $\pistar$ on a certain relevant state of $\pistar$. In the sequel we will prove upper and lower bounds on the intermediate quantity $\sum_{\pistar \in \Pi} \En_0 \brk*{N^\pistar}$ and relate these quantities to $\En_0[\st]$.

\paragraph{Step 1: upper bound.} First we prove an upper bound. We can compute that
\begin{align*}
\sum_{\pistar \in \Pi} \En_0 \brk*{N^\pistar} &= \sum_{t=1}^\Tmax \sum_{\pistar \in \Pi} \En_0 \brk*{\ind{\st > t - 1} \ind{\alg_t(s_{1:H}) = \pistar(s_{1:H}) \wedge s_1 \in \Srel^\pistar}} \\ 
&= \sum_{t=1}^\Tmax \En_0 \brk*{\ind{\st > t - 1} \sum_{\pistar \in \Pi} 
 \ind{\alg_t(s_{1:H}) = \pistar(s_{1:H}) \wedge s_1 \in \Srel^\pistar}}  \\
&\overleq{(i)} \sum_{t=1}^\Tmax \En_0 \brk*{\ind{\st > t - 1} }\\
&\leq \En_0 \brk*{\st \wedge \Tmax} \leq \En_0 \brk*{\st}. \numberthis \label{eq:sum-upper-bound}  
\end{align*}
Here, $(i)$ follows because of Property (3) of \pref{lem:piell-properties}: for every  index $j$ and every $\pistar \in \Piell_j$, each $\pistar$ admits a unique sequence of actions, so any policy which the algorithm runs at time $t$ can match with at most one of the $\pistar$. \gene{the notation is a bit confusing, because the $s_{1:H}$ are not really drawn from from the MDP. need to figure out how to delineate between the states and the indices.}

\paragraph{Step 2: lower bound.} Now we turn to the lower bound. In the sequel we denote $\Pr_{0, \pistar}$ and $\En_{0, \pistar}$ to denote the probability and expectation for the MDP $M_{0, \pistar}$ which has transitions identical to $\pistar$ but all the rewards at level $H$ are $\mathrm{Ber}(1/2)$. We use a change of measure argument.
\begin{align*} 
\En_0 \brk*{N^\pistar} &\overgeq{(i)} \En_{0, \pistar} \brk*{N^\pistar}  - \Tmax \Delta(\Tmax) \\ 
&= \frac{1}{\abs{\Phi}} \sum_{\phi \in \Phi} \En_{0, \pistar, \phi} \brk*{N^\pistar}  - \Tmax \Delta(\Tmax) \\
&\overgeq{(ii)} \frac{1}{10}\cdot \frac{1}{\abs{\Phi}} \sum_{\phi \in \Phi}  \KL{\Pr_{0,\pistar, \phi}^{\cF_{\eta \wedge \Tmax}}}{\Pr_{\pistar, \phi}^{\cF_{\eta \wedge \Tmax}}} - \Tmax \Delta(\Tmax) \\
&\overgeq{(iii)} \frac{1}{10} \cdot \KL{\Pr_{0,\pistar}^{\cF_{\eta \wedge \Tmax}}}{\Pr_{\pistar}^{\cF_{\eta \wedge \Tmax}}} - \Tmax \Delta(\Tmax)
\end{align*}
The inequality $(i)$ follows from a change of measure argument via \pref{lem:change_measure}. Here, $\cF_{\st\wedge\Tmax}$ denotes the natural filtration generated by the first $\st\wedge \Tmax$ episodes. The inequality $(ii)$ follows from \pref{lem:kl-calculation}, using the fact that $M_{0, \pistar}$ and $M_\pistar$ have identical transitions and only differ in rewards at level $H$ for the trajectories which reach the end of a relevant combination. The number of times this occurs is exactly $N^\pistar$. The factor $1/10$ is a lower bound on $\kl{1/2}{3/4}$. The inequality $(iii)$ follows by the convexity of KL divergence.

Now we apply \pref{lem:KL-to-kl} to lower bound the expectation for any $\cF_{\st\wedge \Tmax}$-measurable random variable $Z \in [0,1]$ as 
\begin{align*} 
\En_0 \brk*{N^\pistar} &\geq \kl{\En_{0,\pistar} \brk*{Z}}{\En_{\pistar} \brk*{Z}} - \Tmax \Delta(\Tmax)\\
&\geq (1- \En_{0,\pistar} \brk*{Z}) \cdot \log \prn*{\frac{1}{1-\En_{\pistar} \brk*{Z}}} - \log(2) - \Tmax \Delta(\Tmax),
\end{align*}
where the second inequality follows from the bound $\kl{p}{q} \ge (1-p)\log(1/(1-q)) - \log(2)$.

Now we pick $Z = Z_\pistar := \crl{ \st < \Tmax \wedge \cE(\pistar, \phi, \cA(\cD)) }$ and note that $\En_{\pistar}[Z_\pistar] \geq 1-2\delta$ by assumption. This implies that 
\begin{align*}
\En_0 \brk*{N^\pistar} &\geq (1- \En_{0,\pistar} \brk*{Z_\pistar}) \cdot \log \prn*{\frac{1}{ 2 \delta }} - \log(2) - \Tmax \Delta(\Tmax).
\end{align*}
Another application of \pref{lem:change_measure} gives
\begin{align*}
\En_0 \brk*{N^\pistar} &\geq (1- \En_0 \brk*{Z_\pistar}) \cdot \log \prn*{\frac{1}{ 2 \delta }} - \log(2) - \Tmax \Delta(\Tmax) \log \prn*{\frac{e}{ 2 \delta }}. 
\end{align*}
Summing the above over $\pistar\in\Piell$, we get
\begin{align*}
\sum_{\pistar} \En_0 \brk*{N^\pistar} &\geq \prn*{ \abs{\Piell} - \sum_{\pistar}\En_0 \brk*{Z_\pistar} } \cdot \log \prn*{\frac{1}{ 2 \delta }} - \abs{\Piell} \log(2) - \abs{\Piell} \Tmax \Delta(\Tmax) \log \prn*{\frac{e}{ 2 \delta }}. \numberthis\label{eq:sum-lower-bound-1}
\end{align*}

It remains to prove an upper bound on $\sum_{\pistar}\En_0 \brk*{Z_\pistar}$. We calculate that 
\begin{align*}
\sum_{\pistar}\En_0 \brk*{Z_\pistar} &= \sum_{\pistar}\En_0 \brk*{ \ind{\st < \Tmax \wedge \cE(\pistar, \phi, \cA(\cD))  }} \\
&\leq \sum_{\pistar}\En_0 \brk*{ \ind{ \Pr_\pistar\brk*{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } \ge \frac{\eps}{4} } }   \\ 
&\leq \frac{4}{\eps} \cdot \En_0 \brk*{\sum_{\pistar} \Pr_\pistar\brk*{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } }
\end{align*}
The last inequality is an application of Markov's inequality. \gene{there is some extra measurability justification that is needed here (see the agnostic RL paper pg.~52)}

Now we carefully investigate the sum. The sum can be rewritten as \gene{actually here the decoder doesn't matter since the event only depends on the first state}
\begin{align*}
    &\sum_{\pistar} \Pr_\pistar\brk*{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } \\
    = \quad& \sum_{\pistar} \frac{1}{\abs{\Phi}} \sum_{\phi} \sum_{s_1 \in \cS_1} \Pr_{\pistar, \phi} \brk*{s_1} \Pr_{\pistar, \phi}\brk*{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) ~|~ s_1} \\
    \overeq{(i)} \quad&  \frac{1}{\abs{\Phi}} \sum_{\phi} \frac{1}{\abs{\cS_1}} \sum_{s_1 \in \cS_1} \sum_{\pistar} \Pr_{\pistar, \phi} \brk*{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) ~|~ s_1} \\
    \overeq{(ii)} \quad& \frac{1}{\abs{\Phi}} \sum_{\phi} \frac{1}{\abs{\cS_1}} \sum_{s_1 \in \cS_1} \sum_{\pistar} \ind{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H})}. \numberthis\label{eq:sum-of-indicators}
\end{align*}
The equality $(i)$ follows because regardless of which MDP $M_\pistar$ we are in, the first state is distributed uniformly over $\cS_1$. The equality $(ii)$ follows because once we condition on the first state $s_1$, the probability is either 0 or 1. 

Fix any start state $s_1$. We can write
\begin{align*}
\sum_{\pistar} \ind{ s_1 \in \Srel^\pistar \wedge \cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } = \sum_{\pistar \in \Piell_{\idx(s_1)}} \ind{\cA(\cD)(s_{1:H}) = \pistar(s_{1:H}) } = 1,
\end{align*}
where the second equality uses the fact that on the states $s_{1:H}$, each $\pistar \in  \Piell_{\idx(s_1)}$ behaves differently (Property (3) of \pref{lem:piell-properties}), so $\cA(\cD)$ can match at most one of these behaviors. Plugging this back into Eq.~\pref{eq:sum-of-indicators} we arrive at the bound
\begin{align*}
    \sum_{\pistar}\En_0 \brk*{Z_\pistar} \le \frac{4}{\eps}.
\end{align*}
We now use this in conjunction with Eq.~\pref{eq:sum-lower-bound-1} to arrive at the final bound
\begin{align*}
    \sum_{\pistar} \En_0 \brk*{N^\pistar} &\geq \prn*{ \abs{\Piell} - \frac{4}{\eps}} \cdot \log \prn*{\frac{e}{ 2 \delta }} - \abs{\Piell} \log(2) - \abs{\Piell} \Tmax \Delta(\Tmax) \log \prn*{\frac{e}{ 2 \delta }}. \numberthis\label{eq:sum-lower-bound-2}
\end{align*}

\paragraph{Step 3: putting it all together.}
Combining Eqs.~\pref{eq:sum-upper-bound} and \pref{eq:sum-lower-bound-2} we get
\begin{align*}
    \En_0 \brk*{\st} \ge \prn*{ \abs{\Piell} - \frac{4}{\eps}} \cdot \log \prn*{\frac{1}{ 2 \delta }} - \abs{\Piell} \log(2) - \abs{\Piell} \Tmax \Delta(\Tmax) \log \prn*{\frac{1}{ 2 \delta }}.
\end{align*}
This proves the lemma.\qed

\subsection{Change of measure tools}


\begin{lemma}
\label{lem:change_measure}
Let \(Z \in \brk{0, 1}\) be a  \(\cF_{\Tmax}\)-measurable random variable. Then, for every $\pistar \in \Piell$, 
\begin{align*}
\abs{\En_0 \brk*{Z}  - \En_{0,\pistar} \brk*{Z}} \leq  \Tmax^2 \cdot \frac{2^{H-1}}{\abs{\cS_1}} =: \Delta(\Tmax). 
\end{align*}    
\end{lemma}
\begin{proof} 
First we note that
\begin{align*}
    \abs{ \En_0 \brk*{Z}  - \En_{0,\pistar}\brk*{Z} }\le \mathrm{TV}\prn*{\Pr_0^{\cF_\Tmax}, \Pr_{0, \pistar}^{\cF_\Tmax}} \le \sum_{t=1}^\Tmax \En_0 \brk*{ \mathrm{TV}\prn*{ \Pr_0[\cdot|\cF_{t-1}], \Pr_{0,\pistar}[\cdot|\cF_{t-1}] } }.  
\end{align*} 
Here $\Pr_0[\cdot|\cF_t]$ denotes the conditional distribution of the $t$-th trajectory given the first $t-1$ trajectories (similarly for $\Pr_{0, \pistar}$).\gene{The inequality follows from Q 2.16 in John Duchi's info theory notes.}

Now we examine each term $ \mathrm{TV}\prn*{ \Pr_0[\cdot|\cF_{t-1}], \Pr_{0,\pistar}[\cdot|\cF_{t-1}] } $.
\end{proof} 

\paragraph{Claim.} Given a history $\cF_{t-1}$, random policy $\pi^{(t)}$ which is measurable w.r.t~$\cF_{t-1}$, and sequence \(s_{1:H}\), we have 
\begin{align*}
&\abs{\Pr_{0, \pistar}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) - \Pr_{0}(S_{1:H}^t =  s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1} )} \\
&\leq \frac{1}{\abs{\cS_1}}\ind{s_1 \in \Srel^\pistar, s_1 \in \cF_{t-1}}. 
\end{align*} 

We will use this claim to prove the bound on TV.
\begin{align*}
\mathrm{TV}\prn*{ \Pr_0[\cdot|\cF_{t-1}], \Pr_{0,\pistar}[\cdot|\cF_{t-1}] } &\le \frac{(t-1) \cdot 2^{H-1}}{\abs{\cS_1}},
\end{align*}
since there are at most $t-1$ starting states for which $s_1 \in \cF_{t-1}$.
Therefore we can plug this back in to get a final bound of
\begin{align*}
    \abs{ \En_0 \brk*{Z}  - \En_{0,\pistar}\brk*{Z} } \le \Tmax^2 \cdot \frac{2^{H-1}}{\abs{\cS_1}}.
\end{align*}

\begin{proof}[Proof of claim.]
Notice that we only care if $s_1 \in \Srel^\pistar$ because otherwise $\Pr_{0, \pistar}$ and $\Pr_{0}$ behave identically, which explains the indicator on the RHS of the expression we want to prove.

First we observe that the second term can be exactly calculated as 
\begin{align*}
\Pr_{0}(S_{1:H}^t =  s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1} ) = \frac{1}{\abs{\cS_1}} \cdot \frac{1}{2^{H-1}},
\end{align*}
since the state $s_1$ appears with probability $1/\abs{\cS_1}$ and the transitions in $M_0$ are uniform to the next state in the combination lock, so each sequence is equally as likely.

For the first term $\Pr_{0, \pistar}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1})$, we consider the following decomposition
\begin{align*}
    &\Pr_{0, \pistar}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) \\
    &= \Pr_{0, \pistar}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) \cdot ( \ind{s_1 \notin \cF_{t-1}} + \ind{s_1 \in \cF_{t-1}} )
\end{align*}

We apply the trivial bound for the second term of at most $1/\abs{\cS_1}$.

Now we consider the first term, if we have not seen $s_1$ before, i.e., $s_1 \notin \cF_{t-1}$.
\begin{itemize}
    \item If $\pi^{(t)} = \pistar$ on the index $\idx(s_1)$. In this case we have
    \begin{align*}
        \Pr_{0, \pistar, \phi}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) &= \Pr[s_1 ~|~ s_1 \notin \cF_{t-1}] \cdot \ind{\phi(s_{1:H}) = \mathsf{good}} \\
        &= \frac{1}{\abs{\cS_1}} \ind{\phi(s_{1:H}) = \mathsf{good}},
    \end{align*}
    so we have 
    \begin{align*}
        \Pr_{0, \pistar}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) = \frac{1}{\abs{\cS_1} \cdot 2^{H-1}}
    \end{align*}
    \item Otherwise, $\pi^{(t)}$ deviates from $\pistar$ for the first time at level $h^{(t)}$ so we can write
    \begin{align*}
        \Pr_{0, \pistar, \phi}(S_{1:H}^t = s_{1:H} ~|~ \pi^{(t)}, \cF_{t-1}) &= \Pr_{0, \pistar, \phi}(S_{1:H}^t = s_{1:H}, \pi^{(t)}_{h^{(t)}} \ne \pistar_{h^{(t)}} ~|~ \pi^{(t)}, \cF_{t-1}) \\
        &= \frac{1}{\abs{\cS_1}} \ind{\phi(s_{1:{h^{(t)}}-1}) = \mathsf{good}, \phi(s_{{h^{(t)}}:H}) = \mathsf{bad}} \\
        &= \frac{1}{\abs{\cS_1}} \cdot \frac{1}{2^{H-1}}.
    \end{align*}
\end{itemize}
So putting this together we get the desired bound.
\end{proof}

\begin{lemma}\label{lem:kl-calculation}
Let $\cM$ and $\cM'$ be two MDPs that are identical in transition and differ in the reward distributions, denote $r(s,a)$ and $r'(s,a)$. Assume that for all $(s,a)$ we have $r_h(s,a) \ll r'_h(s,a)$. Then for any stopping time $\st$ with respect to $(\cF^t)_{t\ge 1}$ that satisfies $\Pr_{\cM}[\st < \infty] = 1$,
\begin{align*}
    \KL{\Pr_{\cM}^{I_{\st}}}{\Pr_{\cM'}^{I_{\st}}} = \sum_{s\in\cS} \sum_{a\in \cA} \sum_{h\in[H]} \En_{\cM}[N^\st_{s,a,h}] \cdot \KL{r_h(s,a)}{r'_h(s,a)},
\end{align*}
where $N^\st_{s,a,h} := \sum_{t=1}^\st \ind{(S_h^t, A_h^t) = (s,a) }$ and $I_\st: \Omega \to \cup_{t\ge 1} \cI_t : \omega \mapsto I_{\st(\omega)}(\omega)$ is the random vector representing the history up to episode $\st$.
\end{lemma}

\begin{proof}\gene{this proof is a straightforward modification from Domingues Lemma 5, I wrote enough to verify it is correct for us.}
First we compute the measure under $I_\eta$:
\begin{align*}
    \forall T, \forall i_T \in \cI_T: \Pr_\cM^{I_\eta}[i_T] = \Pr_\cM^{I_T}[\st = T, i_T] = \Pr_\cM[\st = T ~|~ I_T = i_t] \P_\cM^{I_T}[i_T].
\end{align*}
Therefore as long as $\Pr_{\cM'}[\st = T ~|~ I_T = i_t] > 0$ and $\P_{\cM'}^{I_T}[i_T] > 0$ we can compute the ratio of probabilities
\begin{align*}
    \frac{\Pr_\cM^{I_\eta}[i_\eta]}{\Pr_{\cM'}^{I_\eta}[i_\eta]} = \frac{\P_\cM^{I_T}[i_T]}{\P_{\cM'}^{I_T}[i_T]},
\end{align*}
since $\Pr_{\cM}[\st = T ~|~ I_T = i_t] = \Pr_{\cM'}[\st = T ~|~ I_T = i_t]$ as the stopping time event $\crl{\st = T}$ only depends on $I_T$, not on $\cM$ or $\cM'$.

\begin{align*}
    \KL{\Pr_{\cM}^{I_{\st}}}{\Pr_{\cM'}^{I_{\st}}} &= \sum_{T=1}^\infty \sum_{i_T \in \cI_T} \Pr_\cM^{I_\eta}[i_T] \log \prn*{ \frac{\P_\cM^{I_\st}[i_T]}{\P_{\cM'}^{I_\st}[i_T]} } \\
    &= \sum_{T=1}^\infty \sum_{i_T \in \cI_T}  \Pr_\cM[\st = T ~|~ I_T = i_t] \P_\cM^{I_T}[i_T] \log \prn*{ \frac{\P_\cM^{I_T}[i_T]}{\P_{\cM'}^{I_T}[i_T]} } \\
    &\overeq{(i)} \sum_{T=1}^\infty \sum_{i_T \in \cI_T}  \Pr_\cM[\st = T ~|~ I_T = i_t] \P_\cM^{I_T}[i_T] \sum_{t=1}^T \sum_{h=1}^H \log \prn*{ \frac{ r_{h}(s_h^t, a_h^t) }{ r'_{h}(s_h^t, a_h^t) } } \\
    &= \sum_{T=1}^\infty \En_{\cM} \brk*{ \ind{\st = T} \cdot \sum_{t=1}^T \sum_{h=1}^H \log \prn*{ \frac{ r_{h}(s_h^t, a_h^t) }{ r'_{h}(s_h^t, a_h^t) } } } \\
    &= \En_{\cM} \brk*{ \sum_{t=1}^\eta \sum_{h=1}^H \log \prn*{ \frac{ r_{h}(s_h^t, a_h^t) }{ r'_{h}(s_h^t, a_h^t) } } }.
\end{align*}
For equality $(i)$, we use chain rule, the fact that algorithm's decisions cancel, and the fact that the probability transitions are the same.

Now we apply chain rule and use the Markov property:
\begin{align*}
    \KL{\Pr_{\cM}^{I_{\st}}}{\Pr_{\cM'}^{I_{\st}}} &=  \En_{\cM} \brk*{ \sum_{t=1}^\eta \sum_{h=1}^H \En_{\cM} \brk*{\log \prn*{ \frac{ r_{h}(S_h^t, A_h^t) }{ r'_{h}(S_h^t, A_h^t) } }  ~\mid~ S_h^t, A_h^t} } \\
    &=  \En_{\cM} \brk*{ \sum_{t=1}^\eta \sum_{h=1}^H \KL{r_{h}(S_h^t, A_h^t)~}{~r'_{h}(S_h^t, A_h^t)} } \\
    &= \sum_{s,a,h} \En_{\cM}[N_{s,a,h}^\eta] \cdot \KL{r_{h}(s,a)~}{~r'_{h}(s,a)}.
\end{align*}
This concludes the proof.
\end{proof}

\begin{lemma}[Lemma 1, Garivier et al.]\label{lem:KL-to-kl} Consider a measurable space $(\Omega, \cF)$ equipped with two distributions $\bbP_1$ and $\bbP_2$. For any $\cF$-measurable function $Z: \Omega \to [0,1]$ we have
\begin{align*}
    \KL{\bbP_1}{\bbP_2} \ge \kl{\En_1[Z]}{\En_2[Z]}
\end{align*}\gene{add a citation.}
\end{lemma}

==> sections/minimax-complexity.tex <==
\newpage
\section{Towards Minimax Complexity of Agnostic RL} 
Our goal is to understand the minimax sample complexity of agnostic RL. We study learnability in the probably approximately correct (PAC) sense. \gene{I mostly just copied over what I had written before.}  

\subsection{PAC learning}
\begin{definition}[PAC learnability for policy-based RL]
Fix any $\eps,\delta \in (0,1)$. The \emph{sample complexity} of $(\eps,\delta)$-PAC learning a policy class $\Pi$ over MDP class $\wt{\cM}$, denoted $n(\eps, \delta; \Pi, \wt{\cM})$, is defined as the smallest $n \in \bbN$ for which there exists an algorithm $\alg$ such that, for every $M \in \wt{\cM}$, with probability at least $1-\delta$ over the data collection process run by $\alg$, we have
\begin{align*}
    V^\pihat(s_1) \ge \max_{\pi \in \Pi} ~ V^\pi(s_1) - \eps.
\end{align*}
We say $\Pi$ is \emph{PAC learnable} over $\wt{\cM}$ if for all $\eps, \delta \in (0,1)$, $n(\eps, \delta; \Pi, \wt{\cM})$ is finite.
\end{definition}

We study two models of access to a given MDP.
\begin{enumerate}
    \item Online access: the learner can only interact with the MDP by selecting a policy and observing a full episode from the policy. We denote the sample complexity of learning $\Pi$ in this access model as $\non(\eps,\delta;\Pi, \wt{\cM})$.
    \item Generative model access: the learner can transit to any state and query any action. We denote the sample complexity of learning $\Pi$ in this access model as $\ngen(\eps,\delta;\Pi, \wt{\cM})$.
\end{enumerate}

\subsection{\dimname{}: a new complexity measure}
First we will define a notion of reachability for a given policy class $\Pi$ and deterministic MDP $M \in \cMdet$. We denote $\tau_{\pi, M}$ to be the state-action trajectory $\{(s_h, a_h)\}_{h \in [H]}$ that $\pi$ generates on $M$ (that is, $a_h = \pi_h(s_h)$ and $P(s_{h+1}|s_h, a_h) = 1$ for all $h\in [H]$).

\begin{definition}
Fix a deterministic MDP $M \in \cMdet$. We say the state-action pair $(s,a)$ is \emph{reachable} by $\Pi$ if there exists a policy $\pi \in \Pi$ such that $(s,a) \in \tau_{\pi,M}$.
\end{definition}

\begin{definition}[\dimname{}]
Fix a deterministic MDP $M \in \cMdet$. We define the reachability at level $h\in[H]$, denoted $C^\mathsf{reach}_h(\Pi; M)$, as
\begin{align*}
    C^\mathsf{reach}_h(\Pi; M) \coloneqq \abs{ \crl{(s,a): s\in \cS_h, a\in \cA, (s,a) \text{ reachable by } \Pi} }.
\end{align*}
We define the \emph{\dimname{}} of $\Pi$ to be
\begin{align*}
    \dimRL(\Pi) \coloneqq \max_{h \in [H]} \max_{M \in \cMdet} C^\mathsf{reach}_h(\Pi; M).
\end{align*}
\end{definition}

\paragraph{Intuition.} The \dimname{} represents the largest multi-armed bandit instance one can embed in an MDP. This is formalized in the lower bound for deterministic MDPs.

\paragraph{Connection to coverability.}
The \dimname{} is connected to the notions of \emph{coverability coefficient} and \emph{cumulative reachability} defined in the recent work \cite{xie2022role}. For any stochastic MDP $M \in \cMsto$, the coverability coefficient $C^\mathsf{cov}$ is denoted
\begin{align*}
   C^\mathsf{cov}(\Pi; M) \coloneqq~ \inf_{\mu_1, \dots \mu_H \in \Delta(\cS \times \cA)} \sup_{\pi \in \Pi, h \in [H]} ~ \bigg\lVert \frac{d^\pi_h}{\mu_h} \bigg\rVert_\infty =~ \max_{h \in [H]}~ \sum_{s, a} \sup_{\pi \in \Pi} d^\pi_h(s,a).
\end{align*}
The last equality is shown in Lemma 3 of the paper \cite{xie2022role}, and it says that the coverability coefficient is equivalent to cumulative reachability.

In fact, for deterministic MDPs, the definition of reachability coincides: that is, for any $M \in \cMdet$, if $d^\pi_h(s,a)$ is the occupancy measure of $\pi$ in $M$, then $C^\mathsf{reach}_h(\Pi; M) = \sum_{s, a} \sup_{\pi \in \Pi} d^\pi_h(s,a)$. We show that \dimname{} is always an upper bound on coverability, even for any \emph{stochastic} MDP. In other words, the reachability of a policy class is always maximized by a deterministic MDP.

\begin{lemma}\label{lem:coverability}
For any $M \in \cMsto$, we have $C^\mathsf{cov}(\Pi; M) \le \dimRL(\Pi)$.
\end{lemma}

\begin{proof}[Proof of \pref{lem:coverability}.]
Fix any $M \in \cMsto$, as well as $h \in [H]$. Our goal is to prove that 
\begin{align*}
    \Gamma_h \coloneqq \sum_{s, a} \sup_{\pi \in \Pi} d^\pi_h(s,a) \le \max_{M' \in \cMdet} C^\mathsf{reach}_h(\Pi; M').
\end{align*}

We will set up some additional notation. Let us define a \emph{prefix} $\cX$ as any tuple of pairs of the form
\begin{align*}
    (s_1, a_1, s_2, a_2, \dots, s_k, a_k) \text{ or } (s_1, a_1, s_2, a_2, \dots, s_k, a_k, s_{k+1}), \text{ where } k < h.
\end{align*}
We will denote prefix sequences as $\cX = (s_{1:k}, a_{1:k})$ or $ \cX = (s_{1:k+1}, a_{1:k})$ respectively. For any prefix $\cX$ we let $d^\pi_h(s_h, a_h~|~\cX ; M)$ denote the conditional probability of reaching $(s_h, a_h)$ under policy $\pi$ after seeing prefix $\cX$ in MDP $M$, with $d^\pi_h(s_h, a_h~|~\cX ; M) = 0$ if $\pi(s_i) \ne a_i$ for any $i \in [k] \cup \{h\}$ (that is, the visitation probability of $(s_h, a_h)$ is zero if $\pi$ is inconsistent with the trajectory at any point).

Our strategy will be to explicitly compute the quantity $\Gamma_h$ in terms of the dynamics of $M$ and show that we can upper bound it by a ``derandomized'' MDP $M'$ which witnesses $\dimRL(\Pi)$. Let us unroll one step of the dynamics:
\begin{align*}
    \Gamma_h
    &\coloneqq \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi} d^\pi_h(s_h, a_h; M) \\
    &\overset{(i)}{=} \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi} d^\pi_h(s_h, a_h ~|~ s_1 ; M) , \\
    &\overset{(ii)}{=} \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi} \Big\{ \sum_{a_1 \in \cA} d^\pi_h(s_h, a_h~|~s_1, a_1; M) \Big\} \\
    &\le \sum_{a_1 \in \cA} \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi}  d^\pi_h(s_h, a_h ~|~ s_1, a_1; M).
\end{align*}
The equality (i) follows due to the fact that $M$ always starts at $s_1$. The equality (ii) follows from the fact that $\pi$ is deterministic, so there exists exactly one $a' = \pi(s_1) \in \cA$ for which $d^\pi_h(s_h, a_h~|~s_1, a'; M) = d^\pi_h(s_h, a_h~|~s_1 ; M)$, with all other $a'' \ne a'$ satisfying $d^\pi_h(s_h, a_h|s_1, a''; M) = 0$. The inequality follows by taking the supremum inside.

Continuing in this way, we can show that
\begin{align*}
\Gamma_h &\le \sum_{a_1 \in \cA} \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi} \bigg\{ \sum_{s_2 \in \cS_2} P(s_2 | s_1, a_1) \sum_{a_2 \in \cA} d^\pi_h(s_h, a_h ~|~ (s_{1:2}, a_{1:2}); M) \bigg\} \\
&\le \sum_{a_1 \in \cA} \sum_{s_2 \in \cS_2} P(s_2 | s_1, a_1) \sum_{a_2 \in \cA} \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi}  d^\pi_h(s_h, a_h~|~(s_{1:2}, a_{1:2}); M)  \\
&\dots \\
&\le \sum_{a_1 \in \cA} \sum_{s_2 \in \cS_2} P(s_2 | s_1, a_1) \sum_{a_2 \in \cA} \dots \sum_{s_{h-1} \in \cS_{h-1}} P(s_{h-1}| s_{h-1}, a_{h-2}) \sum_{a_{h-1} \in \cA} \\
&\quad\quad \sum_{s_h \in \cS_h, a_h \in \cA} \sup_{\pi \in \Pi}  d^\pi_h(s_h, a_h~|~(s_{1:h-1}, a_{1:h-1}); M).
\end{align*}
Now we examine the conditional visitation $d^\pi_h(s_h, a_h~|~(s_{1:h-1}, a_{1:h-1}); M)$. Observe that it can be rewritten as
\begin{align*}
    d^\pi_h(s_h, a_h~|~(s_{1:h-1}, a_{1:h-1}); M) = P(s_h|s_{h-1}, a_{h-1}) \cdot \ind{\pi(s_i) = a_i \ \forall i \in [h]}.
\end{align*}
Plugging this back into the previous display and taking the supremum inside the sum again we get that 
\begin{align*}
\Gamma_h &\le \sum_{a_1 \in \cA} \dots \sum_{s_{h} \in \cS_{h}} \P(s_{h-1}| s_{h-1}, a_{h-1}) \sum_{a_{h} \in \cA} \sup_{\pi \in \Pi}   \ind{\pi(s_i) = a_i \ \forall i \in [h]} \\
&= \sum_{a_1 \in \cA} \dots \sum_{s_{h} \in \cS_{h}} P(s_{h-1}| s_{h-1}, a_{h-1}) \sum_{a_{h} \in \cA}   \ind{\exists \pi \in \Pi: \pi(s_i) = a_i \ \forall i \in [h]}
\end{align*}
Our last step is to apply ``derandomization'' to the above, simply by taking the supremum over distributions:
\begin{align*}
&\Gamma_h \le \sum_{a_1 \in \cA} \sup_{s_2 \in \cS_2} \sum_{a_2 \in \cA} \dots \sup_{s_{h} \in \cS_{h}} \sum_{a_{h} \in \cA}   \ind{\exists \pi \in \Pi: \pi(s_i) = a_i \ \forall i \in [h]}.
\end{align*}
The right hand side of this inequality is exactly the definition of $\dimRL_h(\Pi)$. In particular, the above process defines the deterministic MDP which maximizes the reachability at level $h$ (that is, the number of state-action pairs for which there exists a policy $\pi \in \Pi$ which reaches the state and plays the correct action). Therefore we know that $\Gamma_h \le \max_{M' \in \cMdet} C^\mathsf{reach}_h(\Pi; M')$ for every $h\in [H]$, and taking the maximum over $h$ concludes the proof of \pref{lem:coverability}.
\end{proof}

\subsection{Deterministic MDPs} 
It is easy to see that \dimname{} exactly characterizes the sample complexity of learning an optimal policy for deterministic MDPs.

\begin{proposition} 
For any $M\in \cMdet$, there exists an algorithm (Policy Elimination) which requires at most $\dimRL(\Pi)$ trajectories to return an optimal policy. Moreover, for any deterministic $\alg$ there exists an $M \in \cMdet$ on which $\alg$ requires at least $\dimRL(\Pi)$ trajectories to return a $1/2$-optimal policy.
\end{proposition}

One can extend this guarantee to the class of MDPs with deterministic transitions and stochastic rewards, call it $\cMdetP$.
\begin{proposition}
For any $\Pi$, the sample complexity of $(\eps,\delta)$-PAC learning $\Pi$ over $\cMdetP$ is \gene{split upper and lower bounds?}
\begin{align*}
     \Omega \Big(\frac{\dimRL(\Pi)}{\eps^2} \cdot \log \frac{1}{\delta} \Big) \le \non(\eps, \delta; \Pi, \cMdetP) \le  O \Big(\frac{\dimRL(\Pi)}{\eps^2} \cdot \log \frac{\dimRL(\Pi)}{\delta}  \Big).
\end{align*}
\end{proposition}
Observe that the lower bound entails a lower bound for PAC learning over $\cMsto$. So bounded \dimname{} is necessary for learnability.

\subsection{Stochastic MDPs with Generative Access Model}
If we allow the learner generative model access, then \dimname{} exactly characterizes the sample complexity of PAC learning.
\begin{proposition}
For any $\Pi$, the sample complexity $(\eps,\delta)$-PAC learning $\Pi$ over $\cMsto$ is \gene{split upper and lower bounds?}
\begin{align*}
    \Omega \Big(\frac{\dimRL(\Pi)}{\eps^2} \cdot \log \frac{1}{\delta} \Big) \le \ngen(\eps, \delta; \Pi, \cMsto) \le  O \Big(\frac{\dimRL(\Pi)}{\eps^2} \cdot \log \frac{\abs{\Pi}}{\delta}  \Big).
\end{align*}
\end{proposition}
The upper bound is proved using the classical \emph{trajectory tree method} \cite{kearns1999approximate}. The lower bound is due to similar reasoning as before.

% \subsection{Online Setting}
% Lower bound from deterministic already applies here, so we want to show an upper bound:
% \begin{conjecture}
% \end{conjecture}

% \begin{enumerate}
%     \item Separation between $C(\Pi)$ vs core-policy set.
% \end{enumerate}


==> sections/old.tex <==
\section{Old Section 3}

\paragraph{Condition 3.}
We say a policy class $\Pi$ satisfies \textbf{Condition 3} with parameters $(K,D)$, if there exists a Markovian policy class $\Pi_{\exp}$ of size $K$ for which the following condition holds: for any $\pi\in \Pi$, there is a set $\mS_\pi$ of $D$ states: $\mathcal{S}_\pi\triangleq\{\bar{s}_{\pi}^{(1)}, \cdots, \bar{s}_{\pi}^{(D)}\}$ such that for any $1\le h_1 < h_2\le H$ and partial trajectory $(s_{h_1}, a_{h_1}, s_{h_1+1}, a_{h_1+1}, \cdots, s_{h_2})$ which satisfies: \gene{Does the definition need $h_2$? One issue may be if the bad state set is actually all the states in level $\mathcal{S}_H$, then it is impossible to define a complete trajectory from $h_1 \to H$. But we still want the definition to say something meaningful about partial trajectories.}

\begin{itemize} 
    \item $a_{h} = \pi(s_h), \forall h_1\le h\le h_2-1$;
    \item $s_{h}\not\in \left\{\bar{s}_{1}, \cdots, \bar{s}_{D}\right\}$ for every $h_1+1\le h\le h_2$,
\end{itemize}
there exists some $\pi_e \in \Pi_{\exp}$ such that 
$$a_{h} = \pi_e(s_h),\quad \forall h_1+1\le h\le h_2-1.$$


\par For every $\pi\in \Pi, s\in\mS$ and some set of states $\mS'$, we further define
$$\bar{d}^\pi(s, \mS')\triangleq \PP^{\pi, M}\left[\tau: \tau\text{ reaches } s \text{ before any other state in }\mS'\right]$$ \gene{sometimes we use this notation even if $s \in \mS'$, so it should be clearer what we mean.} 
\par We will maintain a set of state-policy tuples $U = \{(s, \pi_s)\}$, where we restrict its element to have property  
\begin{enumerate}
	\item each state $s$ only appears in tuples of $U$ once.
	\item for every element $(s, \pi_s)\in U$, \begin{equation}\label{eq-reach} d^{\pi_s, M}(s)\ge \frac{\epsilon}{12D}.\end{equation}	
\end{enumerate}
Initially we set $U = \emptyset$, and we will iteratively grow this set (note that this set $U$ might not contain all of state-policy pairs for which \eqref{eq-reach} holds). \gene{From discussion, maybe we want to include the initial start state and end state in $U$ for notation purposes?} We also notice that if \eqref{eq-reach} holds for every elements in $U$, then the set of different states in those state-action pairs of $U$:
$$U_s \triangleq\{s:\exists \pi, (s, \pi)\in U\}$$
has at most $\frac{C(\Pi)\cdot 2D}{\epsilon}$ elements. \ayush{I think we should just assume wlog that the MDP has a unique start state and end state (and keep the horizon \(H\) instead of \(H+2\) in the proofs).}\gene{You mean $12D$?}

\par At each iteration, we adopt the following sampling process \label{alg-sample} to collect some trajectory samples.

\begin{algorithm}[!htp]
	\caption{$\mathrm{Sampling}(\Pi_{\exp}, U, N_1, N_2)$}\label{alg-sample}
	\begin{algorithmic}[1]
		\For{$i = 1:N_1$}
			\State Sample one policy $\pi'$ from $\mathrm{unif}(\Pi_{\exp})$;
			\State run policy $\pi'$ to collect a trajectory $\tau$;
			\State $\mD_0\leftarrow \mD_0\cup\{\tau\}$;
		\EndFor
		\For{$s\in U_s$}
			\State Let $h$ to be the layer of $s$;
			\State Find $\pi_s$ such that $(s, \pi_s)\in U$;
			\For{$i = 1:N_2$}
				\State Sample one policy $\pi'$ from $\mathrm{unif}(\Pi_{\exp})$;  
				\State run policy $\pi_s$ to layer $h$;
				\If{ \(\pi_s\) reaches $s$} 
					\State run $\pi'$ for rest of layers to collect the trajectory $\tau$
					\State $\mD_s\leftarrow \mD_s\cup\{\tau\}$
				\EndIf
			\EndFor  
		\EndFor 
		\State Return $\mD_0$ and $\mD_s$ for $s\in U_s$ %\ayush{We should probably maintain a different dataset for each \(s \in U_s\). We can actually define a triplet $(s, \pi_s, \mD_s)$.}
	\end{algorithmic}
\end{algorithm}



\par Next, we will adopt these samples to evaluate $d^\pi(s)$ for every $\pi\in\Pi$ and $s\in\mS_\pi$. We will show that either we can evaluate this with error at most $\frac{\epsilon}{2}$, or we can find some $\pi\in\Pi$ and $s\in\mS_\pi$ such that $s\not\in U_s$, and
$$\bar{d}^\pi(s, \SRem{\pi})\ge \frac{\epsilon}{12D}.$$ 
Notice that since $d^\pi(s)\ge \bar{d}^\pi(s, \mS')$ is always true, if we add this $(s, \pi)$ into $U$, it still satisfies the restriction of $U$ given in \eqref{eq-reach}. 

\par We consider the following identifying process in Algorithm \ref{alg-identify} \gene{Question: we don't need to resample $\mD_s$ again in every iteration right? This might improve the sample complexity bound somewhere. \textcolor{blue}{AS: Good question!}} 

\begin{algorithm}[!htp]
	\caption{Identify$(\Pi_{\exp}, N_1, N_2)$}\label{alg-identify}
	\begin{algorithmic}[1]
		\State $U\leftarrow \emptyset$.
		\While{$\mathrm{True}$}
		\State $(\mD_0, \mD_s)\leftarrow \mathrm{Sampling}(\Pi_{\exp}, U, N_1, N_2)$
		\For{$\pi\in \Pi$}
		\State For $s\in\mS_\pi$, as $f_{0\to s}$ defined in \eqref{eq-f-r}, we further let 
		$$\widehat{P}_{0\to s}\leftarrow \frac{|\Pi_{\exp}|}{|\mD_0|}\sum_{\tau\in \mD_0}\frac{\mathbb{1}[\tau \text{ consistent with }\pi\text{ till }s]}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\text{ consistent with }\pi'\text{ till }s]}f_{0\to s}(\tau)$$
		\For{$s\in\SHP{\pi}$} 
			\For{$s'\in\mS_\pi$}
				\State As $f_{s\to s'}$ defined in \eqref{eq-f-r}, we further let
				$$\widehat{P}_{s\to s'}\leftarrow \frac{|\Pi_{\exp}|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\mathbb{1}[\tau \text{ consistent with }\pi\text{ between }s, s']}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\text{ consistent with }\pi'\text{ between }s, s']}f_{s\to s'}(\tau)$$
			\EndFor
		\EndFor
		\For{$\bar{s}\in\SRem{\pi}$}
			\State We construct Markov chain $\widehat{M}_{\mathrm{tab}}$, with its state space to be $\{0, \bar{s}, e\}\cup (\SHP{\pi})$, and transition defined in \eqref{eq-tab}.
		 	\State Calculate the occupancy $\widehat{d}_{\mathrm{tab}}(\bar{s})$ of state $\bar{s}$ of $\widehat{M}_{\mathrm{tab}}$.
			\If{$\widehat{d}_{\mathrm{tab}}(\bar{s})\ge \frac{\epsilon}{12D}$}
				\State $U\leftarrow U\cup(\bar{s}, \pi)$, and run the next \textbf{while} loop (marked as failure)
			\EndIf
		\EndFor
		\EndFor
		\State If for all $\pi\in \Pi$, Line 16 is not ran, then \textbf{break} the \textbf{while} loop.
		\EndWhile
		\State Return $U$.
	\end{algorithmic}
\end{algorithm} 

\begin{algorithm}[!htp]
	\caption{Evaluate$(\Pi_{\exp}, U, N_1, N_2)$}\label{alg-eval}
	\begin{algorithmic}[1] 
		\State $(\mD_0, \mD_s)\leftarrow \mathrm{Sampling}(\Pi_{\exp}, U, N_1, N_2)$
		\For{$\pi\in \Pi$}
		\State Construct $\bar{\mD}_0$ and $\bar{\mD}_s$ from $\mD_0$ and $\mD_s$ by removing all trajectories that pass through some state in $\SRem{\pi}$.  
		\For{$s\in(\SHP{\pi})\cup \{0\}$} 
			\If{$|\bar{\mD}_s|\ge \frac{N_1}{2}$}
				\For{$s'\in(\SHP{\pi})\cup \{e\}$}
					\State As $f_{s\to s'}, R_{s\to s'}$ defined in \eqref{eq-f-r}, we further let
				\begin{align*}
					\widehat{P}_{s\to s'} & \leftarrow \frac{|\Pi_{\exp}|}{|\bar{\mD}_s|}\sum_{\tau\in \bar{\mD}_s}\frac{\mathbb{1}[\tau \text{ consistent with }\pi\text{ between }s, s']}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\text{ consistent with }\pi'\text{ between }s, s']}f_{s\to s'}(\tau),\\
					\widehat{r}_{s\to s'} & \leftarrow \frac{|\Pi_{\exp}|}{|\bar{\mD}_s|}\sum_{\tau\in \bar{\mD}_s}\frac{\mathbb{1}[\tau \text{ consistent with }\pi\text{ between }s, s']}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\text{ consistent with }\pi'\text{ between }s, s']}R_{s\to s'}(\tau).
				\end{align*}
				\EndFor
			\Else
				\State Let $\widehat{P}_{s\to s'} = \mathbb{1}[s' = e]$ and $\widehat{r}_{s\to s'}\equiv 0$.
			\EndIf
		\EndFor
		\State We construct tabular Markov Reward Process $\widehat{M}^{\mathrm{tab}}$ according to $\widehat{P}_{s\to s'}$ and $\widehat{r}_{s\to s'}$, and initial state to be $0$.
		\State Set $\widehat{V}^\pi$ to be the value function of $\widehat{M}^{\mathrm{tab}}$.
		\EndFor
		\State Return $\widehat{V}^\pi$ for all $\pi\in \Pi$.
	\end{algorithmic}
\end{algorithm}



\subsection{Algorithm Concepts}

\iffalse
\ascomment{I have defined the macros:
\begin{align*}
    S_\pi^{\mathrm{HP}}  &= \SHP{\pi} \\ 
    S_\pi^{\mathrm{Rem}} &= \SRem{\pi}.
\end{align*}
to make it easier to read the proof.}  
\fi

Definition of the following tabular Markov Chain $\widehat{M}_{\mathrm{tab}}$: its initial state is $0$, and the transition is \ayush{Should clarify what is $\bar{s}$?}  \gene{This construction is just for the Identify algorithm's construction of $\widehat{M}^\mathrm{tab}$, since the transitions include $\bar{s}$.} 
\begin{equation}\label{eq-tab}
	\begin{aligned} 
		P(s'|s) & = \widehat{P}_{s\to s'} \quad s\in\SHP{\pi}\cup\{0\}, s'\in(\SHP{\pi})\cup{\bar{s}},\\
		P(e|s) & = 1 - \sum_{s'\in (\SHP{\pi})\cup{\bar{s}}} \widehat{P}_{s\to s'} \quad s\in\SHP{\pi}\cup\{0\},\\
		P(e|\bar{s}) & = 1, \quad P(s'|\bar{s}) = 0 \quad \forall s'\in (\SHP{\pi})\cup{\bar{s}},\\
		P(e|e) & = 1, \quad P(s'|e) = 0\quad \forall s'\in (\SHP{\pi})\cup{\bar{s}}.
	\end{aligned}
\end{equation} 
For state $s\in\mS_\pi$ in layer $h$, and state $s'\in\mS_\pi$ in layer $h'$ ($h\le h'$), we define \gene{Should eventually macro-ify and think of best way to do notation.}
\begin{equation}\label{eq-f-r}
	\begin{aligned}
		f_{0\to s}(\tau) & = \mathbb{1}[\tau\text{ reaches }s\text{ before other states in }S_\pi],\\
		f_{0\to e}(\tau) & = \mathbb{1}[\tau\text{ never reaches states in }S_\pi],\\
		f_{s\to s'}(\tau) & = \mathbb{1}[\text{after } s, \tau\text{ reaches }s'\text{ before other states in }S_\pi],\\
		f_{s\to e}(\tau) & = \mathbb{1}[\text{after } s, \tau\text{ never reaches states in }S_\pi],\\
		R_{0\to s}(\tau) & = \mathbb{1}[\tau\text{ reaches }s\text{ before other states in }S_\pi]R(\tau_{0, h}),\\
		R_{0\to e}(\tau) & = \mathbb{1}[\tau\text{ never reaches states in }S_\pi]R(\tau_{0, H}),\\
		R_{s\to s'}(\tau) & = \mathbb{1}[\text{after } s, \tau\text{ reaches }s'\text{ before other states in }S_\pi]R(\tau_{h, h'}),\\
		R_{s\to e}(\tau) & = \mathbb{1}[\text{after } s, \tau\text{ never reaches states in }S_\pi]R(\tau_{h, H}),
	\end{aligned}
\end{equation}
where we use $R(\tau_{h, h'})$ to denote the total reward function of trajectory $\tau$ between layer $h$ and $h'$.

\subsection{Algorithm Analysis}
For this algorithm, we first show that if it returns a failure, then the state-policy pair which causes the failure satisfies large reachability. \gene{Comment: In some sense, this identification algorithm is doing some sort of reachability ``amplification''. One naive approach is to start running $\Pi_\mathrm{exp}$ and then restart it every time you encounter any bad state. Indeed, this will reach every state in the MDP with positive probability, but the probability might be arbitrarily bad (I think the variance compounds or something). So this identification procedure will allow you to identify some policy which is more efficient at reaching the bad states.}
\begin{lemma}
	If at some iteration in Algorithm \ref{alg-identify}, we get a failure with policy $\pi$ and state $\bar{s}$, then we have
	$$\bar{d}^\pi(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{12D}.$$
	If Algorithm \ref{alg-identify} doesn't give failure, then we have for all $\bar{s}\in\SRem{\pi}$, 
	$$\bar{d}^\pi(\bar{s}, \SRem{\pi}) < \frac{\epsilon}{4D}.$$
\end{lemma} 
\begin{proof} 
	We first define the following: \ascomment{Note: $\widehat{P}$ is an empirical version of \(\bar{P}\).} 
	\begin{align*} 
		\bar{P}_{0\to s} & \triangleq \PP^\pi[\tau\text{ reaches }s\text{ before other states in }\mS_\pi],\quad \forall s\in\mS_\pi\\ 
		\bar{P}_{0\to e} & \triangleq \PP^\pi[\tau\text{ reaches no state in }\mS_\pi],\quad \forall s\in\mS_\pi\\
		\bar{P}_{s\to s'} & \triangleq \PP^\pi[\text{after }s, \tau \text{ reaches }s'\text{ before other states in }\mS_\pi|\tau\text{ reaches }s],\\
		&\qquad\qquad\forall s\in\SHP{\pi}, s'\in\mS_\pi
	\end{align*}
	Then we will have
	$$\bar{P}_{0\to s} = \EE^\pi[f_{0\to s}(\tau)] = \sum_{\tau}P^{\IS}(\tau)f_{0\to s}(\tau)\cdot \frac{P^\pi(\tau)}{P^{\IS}(\tau)} = \EE^{\IS}\left[\frac{P^\pi(\tau)}{P^{\IS}(\tau)}f_{0\to s}(\tau)\right].$$
	We further notice that $P^\IS(\tau) = \frac{1}{|\Pi_{\exp}|}\sum_{\pi'\in \Pi_{\exp}} P^{\pi'}(\tau)$. According to Condition 3, we know that for any $\tau$ such that $f(\tau)\neq 0$, there exists some $\pi'\in \Pi_{\exp}$, such that $\tau$ is also consistent with $\pi'$ before $s$. Hence we have 
	$$P^{\pi'}(\tau) = \prod_{h'=1}^{h-1} P(s_{h+1}|s_h, \pi'(s_h)) = \prod_{h'=1}^{h-1} P(s_{h+1}|s_h, \pi(s_h)) = P^\pi(\tau),$$
	where we assume $s = s_h$ is in layer $h$. Therefore, we obtain that
	$$\frac{P^\pi(\tau)}{P^{\IS}(\tau)}f_{0\to s}(\tau) = |\Pi_{\exp}|\cdot\frac{\mathbb{1}[\tau\text{ is consistent with }\pi\text{ in first }h\text{ layers}]}{\sum_{\pi'\in \Pi}\mathbb{1}[\tau\text{ is consistent with }\pi'\text{ in first }h\text{ layers}]}f_{0\to s}(\tau),$$
	which always lies in the interval $[0, |\Pi_{\exp}|]$. Therefore, according to Hoeffding inequality, we have with probability at least $1 - \delta$,
	$$|\widehat{P}_{0\to s} - \bar{P}_{0\to s}|\le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1}}.$$
	Secondly, we notice that for any $s\in U$, the set $|D_s|\ge \frac{N_2\epsilon}{24D} = N_1$ with high probability. \gene{eventually need to make this into a formal lemma.} And similarly, we can also obtain that with probability at least $1 - \delta$,
	$$|\widehat{P}_{s\to s'} - \bar{P}_{s\to s'}|\le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1}}.$$
	Therefore, with probability at least $1 - \delta$, we have for $\forall s\in \SHP{\pi}\cup\{0\}, s'\in\mS_\pi\cup\{e\}$,
	$$|\widehat{P}_{s\to s'} - \bar{P}_{s\to s'}|\le |\Pi_{\exp}|\sqrt{\frac{2\log((D+1)^2/\delta)}{N_1}}.$$
	And if we use $\bar{P}_{s\to s'}$ to construct such a Markov process, then the occupancy of $\bar{s}$ will be exactly $\bar{d}^\pi(\bar{s}, \SRem{\pi})$. Hence according to the tabular MDP algorithm, we will have
	$$|\widehat{d}_{\mathrm{tab}}(\bar{s}) - \bar{d}^\pi(\bar{s}, \SRem{\pi})|\le |\Pi_{\exp}|D\sqrt{\frac{2\log((D+1)^2/\delta)}{N_1}}.$$
	Hence choosing $N_1 = \mathcal{O}\left(\frac{|\Pi_{\exp}|^2D^4}{\epsilon^2}\right)$, we will have
	$$|\widehat{d}_{\mathrm{tab}}(\bar{s}) - \bar{d}^\pi(\bar{s}, \SRem{\pi})|\le \frac{\epsilon}{12D}.$$
	Hence when failure happens, we know that $\widehat{d}_{\mathrm{tab}}(\bar{s})\ge \frac{\epsilon}{6D}$, which indicates that $\bar{d}^\pi(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{12D}$. And if no failure happens, we know that for any $\bar{s}\in \SRem{\pi}$, $\widehat{d}_{\mathrm{tab}}(\bar{s})\le  \frac{\epsilon}{6D}$, which indicates that for any $\bar{s}\in \SRem{\pi}$, $\bar{d}^\pi(\bar{s}, \SRem{\pi})\le \frac{\epsilon}{4D}$. \gene{The notation for $\widehat{d}_\mathrm{tab}$ seems a bit weird to me, but otherwise this lemma is fine.}
\end{proof}


Our next lemma indicates that the \textbf{while} loop in Algorithm \ref{alg-identify} must end in finite number of iterations.
\begin{lemma}
	The \textbf{while} loop can only be ran at most $\frac{12C(\Pi)D}{\epsilon}$ times.
\end{lemma}
\begin{proof}
	We notice that every failures indicates that $\bar{d}^\pi(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{12D}$. Hence
	$$d^{\pi}(\bar{s})\ge \bar{d}^\pi(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{12D}.$$
	Every time we add a $(s, \pi)$ into $U$, we know that $s\not\in U_s$. Hence according to the coverage assumption, we know that there are at most $\frac{12C(\Pi)D}{\epsilon}$ of such $s$. Hence the \textbf{while} loop must end within $\frac{12C(\Pi)D}{\epsilon}$ number of iterations.
\end{proof} 

We next show that if for all $s\in\SRem{\pi}$, we all have
$$\tilde{d}^\pi(s, \SRem{\pi}) < \frac{\epsilon}{4D},$$
then the evaluation algorithm will return a value $\widehat{V}^\pi$ which is $\epsilon$-close to $V^\pi$. \gene{$\tilde{d}$ or $\bar{d}$?}
\begin{lemma}
	If for some $\pi\in \Pi$, and any $s\in \SRem{\pi}$, we have
 $$\tilde{d}^\pi(s, \SRem{\pi}) < \frac{\epsilon}{4D},$$ 
 Then the output $\widehat{V}^{\pi}$ of Algorithm \ref{alg-eval} satisfies that for any $\pi\in \Pi$,
 $$|\widehat{V}^{\pi} - V^\pi|\lesssim \epsilon$$
\end{lemma} 
\begin{proof} 
	For any $s\in\mS_\pi\cup\{0\}$ and $s'\in \mS_\pi\cup\{e\}$, we define
	$$P_{s\to s'} \triangleq \EE^\pi[f_{s\to s'}(\tau)].$$
	Fix a policy $\pi$, we construct a tabular Markov Reward Process $\tilde{M}^{\mathrm{tab}}$ with state space $(\SHP{\pi})\cup\{0, e\}$ as follows: its transition $P$ and reward $r$ are defined as follows: for $s\in\{0\}\cup (\SHP{\pi})$ and $s'\in \SHP{\pi}$.
	$$\tilde{P}_{s\to s'} = P_{s\to s'}, \quad \tilde{R}_{s\to s'} = \EE^\pi[R_{s\to s'}(\tau)]$$
	For $s\in\{0\}\cup (\SHP{\pi})$, we let
	$$\tilde{P}_{s\to e} = 1 - \sum_{s'\in \SHP{\pi}}P_{s\to s'} = P_{s\to e} + \sum_{s'\in \SRem{\pi}}P_{s\to s'},\quad \tilde{R}_{s\to e} = \EE^\pi[R_{s\to e}(\tau)].$$\gene{Something I am confused about: if we directly divide by $|\mD_s|$ in the algorithm (but still do the trajectory deletion stuff) is our estimator unbiased for $\tilde{P}$?}
	We let the value function of $\tilde{M}^{\mathrm{tab}}$ to be $\tilde{V}^\pi$. Then we have our first claim:
	\par \textbf{Claim: } We have
	$$|\tilde{V}^\pi - V^\pi|\le \frac{\epsilon}{4}.$$
	To see this, we first define a reward function $R'$ for trajectory $\tau$ which passes through states in $\SRem{\pi}$: suppose the states in $\mS_\pi$ where $\tau$ passes through are $s_1, s_2, \cdots, s_t$, where we assume $1\le t'\le t$ is the smallest $t$ satisfies that $s_{t'}\in \SRem{\pi}$. We define $R'(\tau) = R(\tau[1:h]) + \tilde{R}_{s_{t'-1}\to e}\in [0, 1]$, where we assume $s_{t'-1}$ is in layer $h$. Then we can write \gene{there should be a probability in these equations.}
	\begin{align*}
		|\tilde{V}^\pi - V^\pi| & = \left|\sum_{\tau}\mathbb{1}[\tau \text{ passes through } \SRem{\pi}]\cdot (R(\tau) - R'(\tau))\right|\\
		&\le \sum_{\tau}\mathbb{1}[\tau \text{ passes through } \SRem{\pi}]\\
		& = \sum_{s\in\SRem{\pi}} \tilde{d}(s, \SRem{\pi})\le \frac{\epsilon}{4D}\cdot D = \frac{\epsilon}{4}.
	\end{align*}
	

	
	\par Next, we bound the difference between $\tilde{V}^\pi$ and $\widehat{V}^\pi$. Assume $\tilde{d}(s)$ to be the occupancy of $s$ in $\tilde{M}^{\mathrm{tab}}$. According to simulation lemma, we have
	$$|\widehat{V}^\pi - \tilde{V}^\pi|\lesssim \sum_{s\in \{0\}\cup(\SHP{\pi})}\tilde{d}(s)\left(\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{P}_{s\to s'} - \widehat{P}_{s\to s'}| + |\tilde{r}_{s\to s'} - \widehat{r}_{s\to s'}|\right),$$
	where $\tilde{d}(s)$ is the occupancy of $s$ in $\tilde{M}^{\mathrm{tab}}$, which coincides with $\tilde{d}(s, \SRem{\pi})$. For $s\in \{0\}\cup(\SHP{\pi})$, and $s'\in \{e\}\cup\{\SHP{\pi}\}$, we define
	$$\bar{P}_{s\to s'}\triangleq \frac{P_{s\to s'}}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}},\quad \bar{r}_{s\to s'}\triangleq \frac{\EE^\pi[R_{s\to s'}(\tau)]}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}},$$
	and we have
	\begin{align*}
		|\tilde{P}_{s\to s'} - \widehat{P}_{s\to s'}| & \le |\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}| + |\bar{P}_{s\to s'} - \widehat{P}_{s\to s'}|
	\end{align*}
	
	\par \textbf{Claim: } We have
	$$\sum_{s\in \{0\}\cup(\SHP{\pi})}\tilde{d}(s)\left(\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}| + |\tilde{r}_{s\to s'} - \bar{r}_{s\to s'}|\right)\lesssim \epsilon$$
	To prove this, we first notice that for $s\in \{0\}\cup (\SHP{\pi})$ and $s'\in \SHP{\pi}$, we have
	$$|\bar{P}_{s\to s'} - \tilde{P}_{s\to s'}| = P_{s\to s'}\left|\frac{1}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}} - 1\right|.$$
	Therefore, we have
	$$\sum_{s'\in \SHP{\pi}}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}| = \left(\sum_{s'\in \SHP{\pi}}P_{s\to s'}\right) \left|\frac{1}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}} - 1\right|\le \left|\frac{1}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}} - 1\right|.$$
	The next thing we notice is that
	$$\tilde{d}(s)\cdot \sum_{s'\in \SRem{\pi}}P_{s\to s'}\lesssim \sum_{s'\in\SRem{\pi}} \tilde{d}(s', \SRem{\pi})\le D\cdot \frac{\epsilon}{4D}\le \frac{\epsilon}{4}.$$
	When $\sum_{s'\in \SRem{\pi}}P_{s\to s'}\ge \frac{1}{2}$, we know that $\tilde{d}(s)\le \frac{\epsilon}{2}$, hence \gene{should this be $\tilde{P} - \bar{P}$?}
	$$\tilde{d}(s)\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{P}_{s\to s'} - \widehat{P}_{s\to s'}|\le 2\tilde{d}(s)\le \epsilon.$$ 
	When $\sum_{s'\in \SRem{\pi}}P_{s\to s'} < \frac{1}{2}$, we know that
	$$\left|\frac{1}{1 - \sum_{s'\in \SRem{\pi}}P_{s\to s'}} - 1\right|\le 2\sum_{s'\in \SRem{\pi}}P_{s\to s'},$$
	which indicates that
	$$\tilde{d}(s)\sum_{s'\in \SHP{\pi}}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}|\le 2\tilde{d}(s)\sum_{s'\in \SRem{\pi}}P_{s\to s'}\le \frac{\epsilon}{2}.$$
	Hence we obtain that
	$$\tilde{d}(s)\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}|\le 2\tilde{d}(s)\sum_{s'\in\SHP{\pi}}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}|\le \epsilon.$$
	Above all, we get
	$$\tilde{d}(s)\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{P}_{s\to s'} - \bar{P}_{s\to s'}|\le\epsilon, \quad \forall s\in\{0\}\cup (\SHP{\pi}).$$ \gene{This is a statement for every $s$. When we sum up all the s, shouldn't we get an extra factor of $D$ in the claim?}
	Similarly, we can also show that
	$$\tilde{d}(s)\sum_{s'\in \{e\}\cup(\SHP{\pi})}|\tilde{r}_{s\to s'} - \bar{r}_{s\to s'}|\le\epsilon, \quad \forall s\in\{0\}\cup (\SHP{\pi}).$$ \gene{For rewards, maybe we need to be a bit more careful? I'm worried there might be some extra factors of $D$}
	
	\par Next, we will analyze the second term related to $|\bar{P}_{s\to s'} - \widehat{P}_{s\to s'}|$. We have the following claim:
	\par \textbf{Claim: } For every $s\in \SHP{\pi}$, if $|\bar{\mD}_s|\le \frac{N_1}{2}$, then with high probability we have $\tilde{d}(s, \SRem{\pi})\le \epsilon$.
	\par To see this, we first notice that $|\mD_s|, |\mD_0|\ge N_1$ happens with high probability if we choose $N_2 = \frac{24N_1 D}{\epsilon}$. If there exists some $s\in \SHP{\pi}$ such that $|\bar{\mD}_s|\le \frac{N_1}{2}$, we use $P^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)}$ to denote the probability of running policy $\pi$ in the original MDP starting from $s$, the probability of never encountering any state in $\mS_\pi$ or the first state we encounter in $\mS_\pi$ (not including $s$ itself) belongs to $\SHP{\pi}$. We use $T_s$ to denote the trajectory starting from $s$, in the future it never encounters any state in $\mS_\pi$ or the first state it encounters in $\mS_\pi$ (not including $s$ itself) belongs to $\SHP{\pi}$. Then we have
	\begin{align*}
		\bar{P}^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)} & = \sum_{\tau} P^\pi(\tau)\mathbb{1}[\tau\in T_s]\\
		& = \sum_{\tau}P^{\IS}(\tau)\cdot \frac{P^\pi(\tau)}{P^{\IS}(\tau)}\mathbb{1}[\tau\in T_s]\\
		& = \mathbb{E}^{\IS}\left[\frac{P^\pi(\tau)}{P^{\IS}(\tau)}\mathbb{1}[\tau\in T_s]\right]\\
		&\le |\Pi_{\exp}|\cdot \mathbb{E}^{\IS}\left[\mathbb{1}[\tau\in T_s]\right].
	\end{align*}
	We further notice that $\sum_{\tau\in D_s}\mathbb{1}[\tau\in T_s] = \bar{D}_s$. \gene{switched to $D_s$ instead of $\mD_s$ notation here.} Hence according to Hoeffiding inequality, we know that with high probability, we have
	$$\left|\frac{|\bar{D}_s|}{|D_s|} - \bar{P}^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)}\right|\lesssim \sqrt{\frac{1}{N_1}}.$$
	Hence if $|\bar{D}_s|\le \frac{N_1}{2}$, we have 
	$$\bar{P}^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)}\le \frac{2}{3}.$$ For $s'\in \SRem{\pi}$, we let $\bar{P}^{\pi, M}_{s\to s'}$ to denote the probability of running policy $\pi$ in the original MDP starting from $s$, the probability of the first state we encounter in $\mS_\pi$ (not including $s$ itself) is $s'$. Then we have
	$$\frac{\epsilon}{4D}\ge \tilde{d}^\pi(s', \SRem{\pi})\ge \tilde{d}(s, \SRem{\pi})\bar{P}^{\pi, M}_{s\to s'}, \quad \forall s'\in\SRem{\pi}.$$
	Sum this up for all $s'\in \SRem{\pi}$, and notice that 
	$$\bar{P}^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)} = 1 - \sum_{s'\in \SRem{\pi}}\bar{P}^{\pi, M}_{s\to s'},$$
	we obtain that
	$$\frac{\epsilon}{4}\ge \tilde{d}(s, \SRem{\pi})\cdot \left(1 - \bar{P}^{\pi, M}_{s\to \{e\}\cup (S_\pi\cap U)}\right)\ge \frac{1}{3}\bar{d}(s, \SRem{\pi}).$$
	Therefore, we obtain that $\tilde{d}(s, \SRem{\pi})\le \epsilon$. Hence either we have $\tilde{d}(s, \SRem{\pi})\le \epsilon$, or we have $|\bar{\mD}_s|\ge \frac{N_1}{2}$.
	\par Next we notice that according to Hoeffding inequality, we have
	\begin{align*}
		|\widehat{P}_{s\to s'} - \bar{P}_{s\to s'}| & \le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{|\bar{D}_s|}}, \\
		|\widehat{r}_{s\to s'} - \bar{r}_{s\to s'}| & \le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{|\bar{D}_s|}},
	\end{align*}
	which indicates that
	\begin{align*}
		&\quad \sum_{s\in\{0\}\cup(\SHP{\pi})}\tilde{d}(s, \SRem{\pi})\cdot \left(\sum_{s'}|\widehat{P}_{s\to s'} - \bar{P}_{s\to s'}| + |\widehat{r}_{s\to s'} - \bar{r}_{s\to s'}|\right)\\
		&\le (4\epsilon)\wedge D\cdot \left(2D|\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1/2}}\right).
	\end{align*} \gene{is there a factor of D in the first term $4\epsilon$ (should it be $\epsilon D^2$)? I'm not exactly sure what the calculation is for this inequality, where did the constant 4 come from?}
 
	Choosing proper $N_1$ will indicates that the above is always less than $4\epsilon$. Hence simulation lemma indicates that
	$$|\widehat{V}^\pi - \tilde{V}^\pi|\lesssim \epsilon.$$
	And we obtain that 
	$$|\widehat{V}^\pi - V^\pi|\lesssim \epsilon,$$
	which finishes the proof.
\end{proof}



==> sections/old_upper_bound_proof_sketch.tex <==
\newpage
\subsection{Older version of state id description}
We assume that \(K\), \(D\), the policy set \(\Picore\), and the states \(\crl{\cS_{\pi}}_{\pi \in \Pi}\) are known to the learner before the start of \pref{alg:main} (note that these can be computed via enumeration). For notational convenience, we additionally define a start state \(s_\top\) (at \(h = 0\)) and end state \(s_\bot\) (at \(h = H+1\)), and let \(\cS_\pi^+ = \cS_\pi \cup \crl{s_\top, s_\bot}\). % Note that the states \(s_\top\) and \(s_\bot\) are not directly used in \pref{alg:main}, but are used in the subroutines \(\evaluate\), \(\sampler\) and \(\DPsolver\) described in the appendix. 

The subroutine $\sampler$ (given in \pref{alg:sample}) is used to collect data that will be used by \(\evaluate\) and \(\DPsolver\) for estimation using IS. \(\sampler\) takes as input a state $s$, policy $\pi_s$ which is guaranteed to reach $s$ with probability at least \(\nicefrac{\epsilon}{12D}\), number of samples $n$ and the set $\Picore$, and returns a dataset \(\cD_s\) of at most \(n\) i.i.d.~trajectories each of which passes through \(s\). The first step in \pref{alg:main} is to collect a dataset $\mD_\top$ of trajectories starting from \(s_\top\) (note that we supple \(\pi_{s_\top} = \mathrm{Null}\) as all trajectories pass through \(s_\top\)).\ayush{This can be shrunk further by removing the definition of \(\sampler\).} which collects trajectories that go through some state $s$. The data collected through here will be used for estimating value functions through importance sampling. The input of \pref{alg:sample} will be state $s$, a policy $\pi_s$ which is guaranteed to reach $s$ with probability at least \(\nicefrac{\epsilon}{12D}\), number of samples $n$ and also the set $\Picore$ defined in \pref{def:core_policy}. If the input $s = s_\top$, the data collector collects $n$ i.i.d.~samples by first uniformly sample $\pi_e$ from $\Picore$ then collect a trajectory according to $\pi_e$. Notice that for $s = s_\top$ the policy $\pi_s$ is useless, hence can be chosen to be $\mathrm{Null}$. For $s\neq s_\top$, we first identify the layer of $s$, then we run $\pi_s$ till this layer. If we exactly encounter state $s$, then we uniformly sample $\pi_e$ from $\Picore$ and collect the rest of trajectory according to $\pi_e$. If not, we just discard the sample. Doing this for $n$ times, these trajectories form the set $\mD_s$. 

\par A main building block used in our algorithm is $\sampler$ (given in \pref{alg:sample}), which collects trajectories that go through some state $s$. The data collected through here will be used for estimating value functions through importance sampling. The input of \pref{alg:sample} will be state $s$, a policy $\pi_s$ which is guaranteed to reach $s$ with probability at least \(\nicefrac{\epsilon}{12D}\), number of samples $n$ and also the set $\Picore$ defined in \pref{def:core_policy}. If the input $s = s_\top$, the data collector collects $n$ i.i.d.~samples by first uniformly sample $\pi_e$ from $\Picore$ then collect a trajectory according to $\pi_e$. Notice that for $s = s_\top$ the policy $\pi_s$ is useless, hence can be chosen to be $\mathrm{Null}$. For $s\neq s_\top$, we first identify the layer of $s$, then we run $\pi_s$ till this layer. If we exactly encounter state $s$, then we uniformly sample $\pi_e$ from $\Picore$ and collect the rest of trajectory according to $\pi_e$. If not, we just discard the sample. Doing this for $n$ times, these trajectories form the set $\mD_s$. In the beginning, the main algorithm will collect a dataset $\mD_0$.

The algorithm maintains two sets \(\cI\) and \(\cT\), that are initialized as \(\crl{s_\top}\) and \(\crl{s_\top, \mathrm{Null}}\) in \pref{line:initialization}. The set \(\cI\) denotes the set of \(\nicefrac{\epsilon}{6D}\) reachable states that the algorithm has discovered so far. \(\cT\) contains tuples of the form \((s, \pi_s)\) for every \(s \in \cI\), where \(\pi_s\) denotes a policy that reaches \(s\) with probability at least \(\nicefrac{\epsilon}{6D}\). The algorithm iteratively grows the set \(\cI\) and \(\cT\) in the while loop from \pref{line:while_loop}-\ref{line:while_loop_end}. 
in which it grows the set $\cI$ and $\cT$, which are both empty in the beginning. The algorithm will first identify those $(s, \pi)$ where $\pi\in \Pi, s\in \mS_\pi$ such that $\pi$ reaches $s$ with probability at least \(\nicefrac{\epsilon}{12D}\). These $(s, \pi)$ pairs will be added into $\cT$ and $s$ will be added into $\cI$. In the meantime, for every $s\in\cI$, \pref{alg:sample} is called in order to get samples which pass through $s$.
Inside this while loop, the algorithm  iterates over all policies \(\pi \in \Pi\) in \pref{line:while_loop_start}. For a \(\pi \in \Pi\), the algorithm first computes, in \pref{line:S_sets_comp}, the set \(\SHP{\pi} = \cS^+_\pi \cap \cI\) as the set of all the states in \(\cS_\pi^+\) that have been discovered so far, and \(\SRem{\pi} = \cS_\pi^+ \setminus \SHP{\pi}\) as the set of remaining states. The algorithm then identifies, in \pref{line:state_identification},  whether there is any \(\bar{s} \in \SRem{\pi}\) that is directly reachable via \(\pi\) (i.e. reachable via trajectories that do not  pass  through any other state in \(\cS_\pi\)) with probability at least \(\nicefrac{\epsilon}{6D}\). If such a state is found, then \((\bar{s}, \pi)\) is added to 
$\cT$ (and \(\bar{s}\) to \(\cI\)) in \pref{line:add_s}, and we continue with the while loop to grow \(\cT\) (or \(\cI\)) further. A fresh dataset $\cD_{\bar{s}}$ is collected in \pref{line:fresh_dataset}.

\ayush{The name of the algorithm is a bit confusing as we identify \(\frac{\epsilon}{4D}\) reachable states and not \(\epsilon\)-reachable states.} 

In order to check whether a state \(\bar{s} \in \SRem{\pi}\) should be added to $\cT$, the algorithm constructs a tabular Markov chain with state space $\mS_\pi^+$, where $s_{\top}$ is in layer $0$ and serves as start state, and $s_{\bot}$ is in layer $H+1$ and serves as the end state. For states $s\in \SHP{\pi}$ and \(s' \in \SRem{\Pi}\), the transition \(P_{s\to s'}^\pi\) is given by:  \ayush{What happens to other transitions outside of these \(s, s'\).} 
\zeyu{Other transitions outside $s, s'$ is not used in evaluating $P_{s\to s'}^\pi$, but they may be useful in other estimations}
\begin{align*} 
 P_{s\to s'}^\pi \ldef{} \Pr^{\pi}\prn*{\tau~\text{goes from \(s\) to \(s'\) without passing through any other state in \(\cS_\pi\)}}.  \numberthis \label{eq:actual} 
\end{align*}
In \pref{line:prob_estimate}, we compute estimates $\widehat{P}_{s\to s'}$ of ${P}_{s\to s'}$ by using importance sampling on dataset $\mD_s$:  
% \begin{equation}\label{eq:empirical}
% 	\widehat{P}_{s\to s'}^\pi = \frac{|\Picore|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\ind{\pi\cons\tau_{h:h'}}}{\sum_{\pi'\in \Picore}\ind{\pi' \cons \tau_{h:h'}}}\ind{\tau\in \event{s}{s'}{\mS_{\pi}}},
% \end{equation} 

\begin{equation}\label{eq:empirical}
	\widehat{P}_{s\to s'}^\pi = \frac{|\Picore|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\ind{\pi\cons\tau_{h:h'}}}{\sum_{\pi'\in \Picore}\ind{\pi' \cons \tau_{h:h'}}}\ind{ \substack{ \text{$\tau_{h:h'}$ goes from \(s\) to \(s'\)} \\ \text{without going through any other \(\cS_\pi\)}}},
\end{equation} 
where for trajectory $\tau = (s_1, a_1, \cdots, s_H, a_H)$ and $s\in \mS_{h}, s'\in\mS_{h'}$, $\tau\in \event{s}{s'}{\bar{\mS}}$ is defined to be the event where $s_{h} = s, s_{h'} = s'$ and for any $h < i < h'$, $s_{i}\not\in \bar{\mS}$. 
With the above estimated-transitions, we compute the probability of directly reaching $\bar{s}\in \SRem{\pi}$ (via trajectories that do not pass through any other \(\cS_\pi\)) by solving the Markov Chain using DP in \ref{line:DP_solver_search}, and if it is large then \(\bar{s}\) is added to \(\cI\) in \pref{line:test_and_add}.

\subsection{Proof Sketch} 

In the following, we provide the technical building blocks for the proof of \pref{thm:sunflower}, and defer the exact details to \pref{app:upper_bound_main}. We run $\mathsf{POPLER}$ using the following choice of parameters 
\begin{align*} 
n_1 = \widetilde{\cO}\prn*{\tfrac{(D^4+1)K^2}{\epsilon^2} \log(|\Pi|/\delta)}, \qquad n_2 = \widetilde{\cO}\prn*{\tfrac{D^5K^2}{\epsilon^3} \log(|\Pi|/\delta }. \numberthis \label{eq:alg_params_informal} 
\end{align*}


\ascomment{\begin{enumerate}
    \item Motivation why we are even looking at \(\cI\), why we hope for reachable states to be bounded. 
    \item Convey why importance sampling alone is not enough for tabular MDPs. 
\end{enumerate}}


\pref{alg:main} first interacts with the MDP to  identify the set \(\cI\) of states (from lines \ref{line:while_loop}-\ref{line:while_loop_end}), each of which is reachable with probability at least \(\nicefrac{\epsilon}{12D}\). In order to grow \(\cI\), the algorithm checks whether there is any policy \(\pi \in \Pi\) for which there is a reachable state in \(\cS_\pi\) that is not yet included in \(\cI\).  Recall that \(\SHP{\pi} = \cS_\pi^+ \cap \cI\) and \(\SRem{\pi} = \cS_\pi^+ \setminus \SHP{\pi}\). For a particular choice of \(\cI\) and \(\pi\), these new states are discovered by constructing a tabular Markov chain for \(\pi\) as described in \pref{sec:algorithm_description} over the state space \(\cS_\pi^+\). The transition probability for this tabular Markov chain is given by \( P_{s\to s'}^\pi\), where for any \(s \in \SHP{\pi}\) and \(s' \in \SRem{\pi}\),
\begin{align*} 
 P_{s\to s'}^\pi \ldef{} \Pr^{\pi}\prn*{\tau~\text{goes from \(s\) to \(s'\) without passing through any other state in \(\cS_\pi\)}}. 
 %, \quad \forall s\in \{0\}\cup \SHP{\pi}, s'\in \mS_\pi\cup\{e\}.
\end{align*}
Our first technical result states that the transition probability estimated in \pref{line:prob_estimate} of \pref{alg:main} closely approximates its true value.  \ayush{I think we need to discuss further here on what this tabular MDP is doing! I think the high-level idea about this tabular MDP is still a bit elusive.} 

% Our proof relies on the following three lemmas. The first lemma indicates that the error of importance sampling can be bounded if with enough samples. 

\begin{lemma}[Informal] 
\label{lem:dynamics_error} For any \(\pi\), states \(\cI\), \(\SHP{\pi}\) and \(\SRem{\pi}\), with probability at least \(1 - \delta\), for all \(s \in \SHP{\pi}\) and \(s' \in \SRem{\pi}\), the estimate \(\wh P_{s\to s'}^\pi\) in \pref{line:prob_estimate} of \pref{alg:main} satisfies %\(       \abs{P_{s\to s'}^\pi - \widehat{P}_{s\to s'}^\pi} \le \widetilde{\cO}\prn*{\tfrac{\epsilon}{(D + 1)^2}}.\) 
    \begin{align*}
       \abs{P_{s\to s'}^\pi - \widehat{P}_{s\to s'}^\pi} \le \widetilde{\cO}\prn*{\tfrac{\epsilon}{(D + 1)^2}}. \numberthis \label{eq:error}
\end{align*}
\end{lemma}

% \begin{lemma}[Informal]
% \label{lem:dynamics_error} 
%     Given that $|\mD_s|\ge \frac{\epsilon n_2}{24D}$ for all $s\in U_{s}$, there exists two universal constants $C_1, C_2$ such that if we choose  
%     $$n_1 = \frac{C_1(D+1)^4K^2\log(|\Pi|(D+1)/\delta)}{\epsilon^2}, n_2 = \frac{D^3(D+1)^2K^2\log(|\Pi|(D+1)^2/\delta)}{\epsilon^3},$$
%     then with probability at least $1 - \delta$, we have $\forall \pi\in\Pi$
%     $$\begin{aligned}\label{eq:error}
%         \left|P_{s\to s'}^\pi - \widehat{P}_{s\to s'}^\pi\right|\le \frac{\epsilon}{12D(D+1)}, &\quad \forall s\in\SHP{\pi}, s'\in \mS_\pi\cup\{e\}\\
%         \left|P_{0\to s'}^\pi - \widehat{P}_{0\to s'}^\pi\right|\le \frac{\epsilon}{12(D+1)^2}, &\quad \forall s'\in \mS_\pi\cup\{e\}\\
%     \end{aligned}$$
%     where $P_{s\to s'}, r_{s\to s'}$ are defined as
%     $$P_{s\to s'}^\pi \triangleq P^{\pi, M}[\tau: \tau\in \event{s}{s'}{\mS_{\pi}}|s\in\tau], \quad \forall s\in \{0\}\cup \SHP{\pi}, s'\in \mS_\pi\cup\{e\}.$$
% \end{lemma}

Having constructed a tabular Markov process as shown in \pref{lem:dynamics_error}, one can simply discover any remaining reachable states by solving Dynamic Programming in \pref{line:DP}. If such a state is found, it is added to \(\cI\). Our next technical lemma concerns with the termination of the  while loop from lines \ref{line:while_loop}-\ref{line:while_loop_end}, and the set \(\cI\) discovered after termination. \ayush{Give more intuition on this tabular MDP.}

The second lemma bounds the number of rounds of the while loop, and also shows that the reachability of states outside $\cI$ is small. This is because every state in some $\mS_\pi$ with large reachability will eventually been put into $\cI$. And $\dimRL(\Pi)$ upper bounds the coverage of $\Pi$, hence also the number of states with large reachability. \ayush{Say that this is exactly where \(C(Pi)\) comes in.} 

\begin{lemma}[Informal] 
\label{lem:while_terminate}
The while loop from lines \ref{line:while_loop}-\ref{line:while_loop_end} in \pref{alg:main} terminates after $O\prn*{\nicefrac{D\dimRL(\Pi)}{\epsilon}}$ iterations. Furthermore, after termination, for any \(\pi \in \Pi\) and \(\bar s \in \prn{\cS_{\pi} \setminus \cI}$, 
\begin{align*}
\Pr^{\pi}\prn*{\tau~\text{goes to \(\bar s\) without passing through any other state in \(\cS_\pi\)}} \leq O\prn*{\tfrac{\epsilon}{D}}. 
\end{align*} 

% $s\in\SRem{\pi} = \mS_\pi\backslash \cI$ we have 
%     $$\bar{d}^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{4D},$$
%     where $\bar{d}^{\pi}(s, \bar{S})\triangleq P^{\pi, M}[\tau: \tau\in \event{0}{s}{\bar{S}}], \forall s, \pi, \bar{S}\subset \mS$.
\end{lemma} 
After discovering all the relevant reachable states \(\cI\), the following lemma shows that for any \(\pi \in \Pi\), the estimated value $\widehat{V}^\pi$ on \pref{line:evaluate} of \pref{alg:main} closely approximates the value of the policy $V^\pi$ in the underlying MDP. This is because the reachability of states in $\SRem{\pi}$ is small, and so transitions and rewards between these states would not have a large influence on value. Thus, ignoring them,  we can approximate \(V^\pi\) by solving a corresponding Tabular Markov Reward Process on \(\SHP{\pi}\).

% don't have large influence. Given that, the key idea behind the proof of the following lemma is that  with enough samples in \(\cD_s\),

% % Our final lemma indicates that if the reachability of states in $\SRem{\pi}$ are all very small, then $\widehat{V}^\pi$ is close to the true value function $V^\pi$. 

% The key idea behind the proof is that 

% for any \(\pi\), with enough samples in \(\cD_s\), we can approximate \(V^\pi\) by solving a corresponding Tabular Markov Reward Process on \(\SHP{\pi}\). Since the  that approximates the value of the policy; secondly, 



\begin{lemma}[Informal]
\label{lem:eval_error}
Suppose the set \(\cI\) satisfies the condition in \pref{lem:while_terminate}. Then, for any \(\pi \in \Pi\), the output of $\widehat{V}^\pi$ in \pref{line:evaluate} in \pref{alg:eval} satisfies $\abs{\widehat{V}^\pi - V^\pi}\le O(\epsilon)$. 
\end{lemma}


\begin{proof}[Proof sketch for \pref{thm:sunflower}]  %The proof follows by a straightforward combination of the above lemmas.
Note that 
 \pref{lem:while_terminate} and \pref{lem:eval_error} together indicate that after  the termination of the while loop, the estimates values satisfy $\abs{\widehat{V}^\pi - V^\pi} \le \epsilon$, and thus the returned policy \(\wh \pi\) in \pref{line:return} satisfies \(V^{\wh \pi} \geq \max_{\pi \in \Pi} V^\pi - O(\epsilon)\). The provided sample complexity bound follows by plugging in the bound on the number of iterations in \pref{lem:while_terminate}, and the value of the parameters \(n_1\) and \(n_2\) from \pref{eq:alg_params_informal}. 
  % indicates that the while loop runs at most $\nicefrac{12D\dimRL(\Pi)}{\epsilon}$ rounds. If we choose $n_1, n_2$ in \pref{lem:dynamics_error}, each $\widehat{V}^\pi$ will be $\epsilon$-close to $V^\pi$. Therefore, the policy with largest $\widehat{V}^\pi$ is an $\epsilon$-optimal policy.
\end{proof}


==> sections/structural.tex <==
\section{Structural assumptions for Agnostic RL}

\subsection{Structural Assumptions} 
\subsubsection{Core Policy Set} 

\begin{assumption}[Core-policy set]   \label{ass:core_policy} 
    We say a policy class $\Pi$ satisfies the \textbf{Core-policy set assumption} with parameters $(K,D)$, if there exists a Markovian policy class $\Pi_{\exp}$ of size $K$ for which the following condition holds: for any $\pi\in \Pi$, there is a set $\mS_\pi$ of $D$ states: $\mathcal{S}_\pi\triangleq\{\bar{s}_{\pi}^{(1)}, \cdots, \bar{s}_{\pi}^{(D)}\}$ such that for any $1\le h_1 < h_2\le H$ and partial trajectory $(s_{h_1}, a_{h_1}, s_{h_1+1}, a_{h_1+1}, \cdots, s_{h_2})$ which satisfies:

\begin{itemize} 
    \item $a_{h} = \pi(s_h), \forall h_1\le h\le h_2-1$;
    \item $s_{h}\not\in \left\{\bar{s}_{1}, \cdots, \bar{s}_{D}\right\}$ for every $h_1\le h\le h_2$,
\end{itemize}
there exists some $\pi_e \in \Pi_{\exp}$ such that 
$$a_{h} = \pi_e(s_h),\quad \forall h_1+1\le h\le h_2-1.$$
\end{assumption}

Some intuition for this assumption? Sort of captures bias-variance tradeoff of nonadaptive sampling.


Example of policy class: 
\begin{enumerate}[label=\(\bullet\)] 
    \item Tabular MDP: 
    \item Contextual Bandit: 
    \item K-tons:
    \item Rich observation K-tons: (shows that we should use nonMarkovian)
    \item \(\Pi_1\): 
    \item \(\Pi^\cup\): 
\end{enumerate}

\begin{lemma}[Limitations of Assumption~\ref{ass:core_policy}] Assumption~\ref{ass:core_policy}  is not enough on its own. 
    
\end{lemma}

\subsubsection{Coverage}
For any policy $\pi$, we define the occupancy $d^\pi(s)$ of state $s$ (of layer $h$) as
$$d^{\pi}(s)\triangleq \mathbb{P}^{\pi, M}[\tau: \tau\text{ passes through }s],$$
where $M$ is the underlying MDP.
\begin{assumption}[Coverability] \label{ass:coverage} 
	We say that the coverage of policy set $\Pi$ under MDP $M$ is bounded by $C(\Pi, M)$, if
	$$\sum_{s\in\mS} \sup_{\pi\in\Pi}d^{\pi, M}(s)\le C(\Pi, M).$$
\end{assumption}

Notice that this assumption was also used in~\cite{xie2022role}.


\begin{enumerate} 
    \item Cite the coverage paper + talk about connections?
    \item Coverability is necessary, but not sufficient.
\end{enumerate}

\subsection{Algorithm} 
\par To facilitate the description of the algorithm, we make the following notations: for any trajectory $\tau$, and any two states $s\in \mS_{h_1}, s'\in \mS_{h_2}$ in $\tau$ with $h_1 < h_2$, we denote $\tau[s:s'] = (s_{h_1}, a_{h_1}, \cdots, s_{h_2})$. We use $\tau[s:s']\sim \pi$ to denote the event that $\tau$ is consistent with $\pi$ between $s$ and $s'$.

We further define the following events: for any trajectory $\tau = (s_1, a_1, \cdots, s_H, a_H)$, $s\in \mS_{h_1}, s'\in\mS_{h_2}$ and $\bar{\mS}\subset \mS$, we say
$$\tau\in \event{s}{s'}{S}$$
if $s_{h_1} = s, s_{h_2} = s'$, and for any $h_1 < h < h_2$, $s_{h}\not\in \bar{\mS}$. If $h_1\ge h_2$, $\event{s}{s'}{\bar{\mS}}$ will always be empty. We further define cases when $s = 0$, $\tau\in \event{s}{s'}{S}$ if and only if $s_{h_2} = s'$ and for any $h < h_2$, $s_h\not\in \bar{\mS}$; and also when $s' = e$, $\tau\in \event{s}{s'}{S}$ if and only if $s_{h_1} = s$ and for any $h > h_1$, $s_h\not\in \bar{\mS}$.

\subsubsection{Ideas of the Algorithm}
\par Suppose \pref{ass:core_policy} holds, we can identify $\Pi_{\exp}$ and $\mS_\pi$ for $\forall \pi\in\Pi$ by just looking at the policy class, without using any samples. In the following, we assume that $\Pi_{\exp}$ and also $\mS_\pi$ are given to us.

\par The idea of the algorithm follows from the importance sampling algorithm. If $D = 0$, i.e. for any trajectory $\tau$ which is consistent with $\pi\in \Pi$ there exists some $\pi_e\in \Pi_{\exp}$ such that $\tau$ is also consistent with $\pi_e$, then adopting importance sampling algorithm: (1) sample $\pi_e\in \Pi_{\exp}$ uniformly; (2) collect a trajectory $\tau$ according to $\pi_e$, and
$$\frac{\mathbb{1}[\tau\sim\pi]}{\frac{1}{|\Pi_{\exp}|}\sum_{\pi_e\in \Pi_{\exp}}\mathbb{1}[\tau\sim\pi_e]}V[\tau]$$
will be an unbiased estimator of $V^{\pi}$. Hence by collecting enough such samples, the law of large number will guarantee an accurate enough estimation of $V^{\pi}$. 

\par When $D > 0$, the importance sampling algorithm does not work directly. To evaluate $V^\pi$, what we hope is that we can form a tabular Markov Reward Process (MRP) with the state space to be $\mS_\pi$, and with the importance sampling algorithm we can evaluate the transition and rewards between states. However, since different policies have different $\mS_\pi$, there so many such states that we cannot afford to collect samples from all of them. 

\par To resolve this, we maintain a state-policy set $U = \{(s, \pi_s)\}$ where $s\in \mS_{\pi_s}$ and the occupancy $d^{\pi_s}(s)$ has a uniform lower bound. Hence \pref{ass:coverage} guarantees that the size of $U_s = \{s:\exists \pi_s, (s, \pi_s)\in U\}$ is bounded. And in the evaluation process, we only form the tabular MRP with the state space to be $\SHP{\pi} = \mS_{\pi}\cap U_s$, and remove the states in $\SRem{\pi} = \mS_\pi\backslash U_s$. In this MRP, only using trajectories generated according to $\pi_s$ (which arrive at $s$ with certain probability) will be enough for importance sampling on $s\in U_s$. Additionally, it can also be shown that removing those states in $\SRem{\pi}$, the influence to $V^{\pi}$ is very small (otherwise the occupancy to those states will be large and we will have to put them into $U$).

\subsubsection{Algorithm Details}
\par Our algorithm (\pref{alg:main}) includes two parts: the \textbf{Identification} part and also \textbf{Evaluation} part. During the identification part, the algorithm identifies those states in some $\mS_\pi$ with high occupancy. Those are states which require additional training. The algorithm will mark those states and also the policy corresponding to it for future training uses. After the identification part, the algorithm goes to the evaluation part, where we use those identified states and policies to evaluate the value functions of policies in the policy set and pick the best one. 
\begin{algorithm}[!htp]
	\caption{Algorithm}\label{alg:main}
	\begin{algorithmic}[1]
		\State Find $\Pi_{\exp}$ and $\mS_\pi$ for every $\pi\in\Pi$.
		\State $\text{Identify}(\Pi_{\exp}, N_1, N_2)$.
		\For{$\pi\in \Pi$}
			\State $\hV^\pi\leftarrow \text{Evaluate}(\pi, \Pi_{\exp}, \mD_0, \mD_s, U, \pi)$
		\EndFor
		\State Return $\widehat{\pi} = \argmax_\pi \hV^\pi$.
	\end{algorithmic}
\end{algorithm}

\par The \textbf{Identification} algorithm (\pref{alg:identify}) aims to find a set $U$ of state-policies such that the following two properties hold: if we define $U_s = \{s:\exists \pi, (s, \pi)\in U\}$, 
\begin{enumerate}
	\item for any $(s, \pi_s)\in U$, we have $d^{\pi}(s)\ge \frac{\epsilon}{12D}$;
	\item for any $\pi\in \Pi$ and $s\in \SRem{\pi}\triangleq \mS_\pi\backslash U_s$, we have $\bar{d}^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{12D}$,
\end{enumerate}
where for any $s\in \mS, \pi\in \Pi$ and subset $\bar{S}\subset \mS$,
$$\bar{d}^{\pi}(s, \bar{S})\triangleq \mathbb{P}^{\pi, M}[\tau: \tau\in \event{0}{s}{\bar{S}}].$$

\par To achieve this goal, we add elements into $U$ iteratively. Initially, $U$ is the empty set. At each iteration, given the current $U$, we will check for any policy $\pi\in \Pi$ and $\bar{s}\in \SRem{\pi}$, whether we have
\begin{equation}\label{eq:srem}\bar{d}^{\pi}(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{12D}.\end{equation}
If none of such policy and state exists, the current $U$ is desirable. And if not, we add those state-policy pair $(\bar{s}, \pi)$ which violate the above inequality into $U$. It is easy to see that $\bar{d}^{\pi}(s, \bar{S})\le d^{\pi}(s)$ for all $s, \pi, \bar{S}$. Hence after adding those state-policy pairs, the first property still holds for $U$. To check whether $\eqref{eq:srem}$ holds for $\pi\in \Pi$ and $\bar{s}\in \SRem{\pi}$, we construct a tabular Markov Chain $\Mtab^{\pi}$ with state space to be $\{0, e\}\cup \mS_\pi$, initial state to be $0$, and transition to be
\begin{equation}\label{eq:original}
\begin{aligned}
	P_{s\to s'} & = \PP^{\pi, M}[\tau: \tau\in \event{s}{s'}{\mS_{\pi}}], \quad \forall s\in \{0\}\cup \SHP{\pi}, s'\in \mS_\pi\cup\{e\}\\
	P_{s\to s'} & = \mathbb{1}[s' = e], \quad \forall s = \SRem{\pi}\cup\{e\}.
\end{aligned}
\end{equation}
We can see (will prove later) that for any $\bar{s}\in \SRem{\pi}$, the occupancy $d^{\Mtab^{\pi}}(\bar{s})$ of $\bar{s}$ under Markov chain $\Mtab^{\pi}$ is exactly $\bar{d}^{\pi}(\bar{s}, \SRem{\pi})$. Therefore, if we can empirically calculate each value of $P(s'|s)$, then we can approximate the occupancy of $\bar{s}$. However, the problem of this scheme is that, directly calculating the empirical transitions of the above Markov chain with respect to all policies requires at least $|\Pi|$ number of samples. And how to reuse samples by adopting importance sampling is one of the key innovation of the algorithm.

\par To avoid number of samples going linearly with $|\Pi|$, we first adopt a sampling scheme (\pref{alg:sample}) given the current $U$ to collect dataset $(\mD_0, \mD_s)$. The sampling procedure collect bunch of trajectories according to a policy uniformly sampled from $\Pi_{\exp}$ to form $\mathcal{D}_0$ (line 1-4). Next for every $s\in U_s$, first we run $\pi_s$ (where $(\pi_s, s)\in U$). If the trajectory reaches $s$ (later we will prove that this happens with a certain probability), then we uniformly sample a policy from $\Pi_{\exp}$ and run that policy for the rest of layers to collect a trajectory; otherwise we discard the samples. Trajectories collected during this process form the dataset $\mathcal{D}_s$.

\begin{algorithm}[!htp]
	\caption{$\mathrm{Sampling}(\Pi_{\exp}, s, \pi_s, N)$}\label{alg:sample}
	\begin{algorithmic}[1]
		\State Suppose $s\in\mS_h$ (for $s = 0$ we let $h = 0$);
		\For{$n = 1:N$}
			\State run policy $\pi_s$ to layer $h$ (for $s = 0$ we do not need $\pi_s$ and the next If always holds);
			\If{ \(\pi_s\) reaches $s$}
				\State Sample $\pi'\sim\mathrm{unif}(\Pi_{\exp})$;  
				\State run $\pi'$ from layer $h$ to $H$ to collect $\tau$;
				\State $\mD_s\leftarrow \mD_s\cup\{\tau\}$;
			\EndIf
		\EndFor  
		\State Return $\mD_s$.
	\end{algorithmic}
\end{algorithm}

\iffalse
\begin{algorithm}[!htp]
	\caption{$\mathrm{Sampling}(\Pi_{\exp}, U, N_1, N_2)$}\label{alg:sample}
	\begin{algorithmic}[1]
		\For{$i = 1:N_1$}
			\State Sample one policy $\pi'$ from $\mathrm{unif}(\Pi_{\exp})$;
			\State run policy $\pi'$ to collect a trajectory $\tau$;
			\State $\mD_0\leftarrow \mD_0\cup\{\tau\}$;
		\EndFor
		\For{$s\in U_s$}
			\State Let $h$ to be the layer of $s$;
			\State Find $\pi_s$ such that $(s, \pi_s)\in U$;
			\For{$i = 1:N_2$}
				\State Sample one policy $\pi'$ from $\mathrm{unif}(\Pi_{\exp})$;  
				\State run policy $\pi_s$ to layer $h$;
				\If{ \(\pi_s\) reaches $s$} 
					\State run $\pi'$ for rest of layers to collect the trajectory $\tau$
					\State $\mD_s\leftarrow \mD_s\cup\{\tau\}$
				\EndIf
			\EndFor  
		\EndFor 
		\State Return $\mD_0$ and $\mD_s$ for $s\in U_s$ %\ayush{We should probably maintain a different dataset for each \(s \in U_s\). We can actually define a triplet $(s, \pi_s, \mD_s)$.}
	\end{algorithmic}
\end{algorithm}
\fi

\par Next, fixed any policy $\pi$, we adopt the importance sampling according to $(\mD_0, \mD_s)$ to form an empirical version of the transition of tabular Markov Chain $\Mtab^{\pi}$: for $\forall s\in \{0\}\cup \SHP{\pi}, s'\in \mS_\pi\cup\{e\}$:\begin{equation}\label{eq:tab}
	\begin{aligned}
		\widehat{P}_{s\to s'}^\pi & = \frac{|\Pi_{\exp}|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\mathbb{1}[\tau[s, s']\sim \pi]}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]}\mathbb{1}[\tau\in \event{s}{s'}{\mS_{\pi}}]\\
		\widehat{r}_{s\to s'}^\pi & = \frac{|\Pi_{\exp}|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\mathbb{1}[\tau[s, s']\sim \pi]}{\sum_{\pi'\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]}\mathbb{1}[\tau\in \event{s}{s'}{\mS_{\pi}}]R(\tau[s:s'])\\
		\widehat{P}_{s\to s'} & = \mathbb{1}[s' = e], \quad \forall s = \SRem{\pi}\cup\{e\}.
	\end{aligned}
\end{equation}
We further notice that if we denote $0\in \mS_0$ and $e\in\mS_{H+1}$, then for any $s\in \mS_{h_1}$ and $s'\in\mS_{h_2}$ where $h_1\ge h_2$, we will have $\widehat{P}_{s\to s'} = 0$. The output will be 

\par With this empirical tabular Markov Chain, we can calculate the empirical estimation $\widehat{d}(\bar{s}$ of $d^{\Mtab^{\pi}}(\bar{s})$ using dynamical programming (\pref{alg:dyna}), with state space to be $\mS_\pi\cup \{0, e\}$, transition to be $P_{s\to s'} = \widehat{P}_{s\to s'}$ and reward to be $r_{s\to s'} = \mathbb{1}[s = \bar{s}, s' = e]$. We know that if the transition is chosen to be \eqref{eq:original}, then the output is exact $\bar{d}^{\pi}(\bar{s}, \SRem{\pi})$, and if with enough samples, the transitions $\widehat{P}$ will close to the transition in \eqref{eq:original}. Therefore, we can identify those $(s, \pi)$ pair where \eqref{eq:srem} holds.

\begin{algorithm}
\caption{DP$(\mS, P, r)$}\label{alg:dyna}
	\begin{algorithmic}
		\State \textbf{Input: } Finite State Space $\mS^{\mathrm{tab}}$, transition $P_{s\to s'}$ and reward $r_{s\to s'}$;
		\State Set $V(s)\equiv 0$ for $\forall s\in \mS_{H+1}$.
		\For{$h=H:0$}
			\State For $\forall s\in\mS_h$, calculate $V(s)\leftarrow \sum_{s'\in\mS^{\mathrm{tab}}} P_{s\to s'}\left(r_{s\to s'} + V(s')\right).$
		\EndFor
		\State \textbf{Output: } $V(0)$.
	\end{algorithmic}
\end{algorithm}



\begin{algorithm}[!htp]
	\caption{Identify$(\Pi_{\exp}, N_1, N_2)$}\label{alg:identify}
	\begin{algorithmic}[1]
		\State $U\leftarrow \emptyset$.
		\State $\mD_0\leftarrow \mathrm{Sampling}(\Pi_{\exp}, 0, \pi_0, N_1)$
		\While{$\mathrm{True}$}
		\For{$\pi\in \Pi$}
			\State Calculate $\widehat{P}_{s\to s'}$ for $s\in\SHP{\pi}\cup\{0\}, s'\in \mS_\pi\cup\{e\}$ according to \eqref{eq:tab}.
			\For{$\bar{s}\in\SRem{\pi}$}
		 		\State Let $\widehat{d}(\bar{s})\leftarrow \text{DP}(\mS_\pi\cup\{0, e\}, \widehat{P}_{s\to s'}, \mathbb{1}[s = \bar{s}])$.
				\If{$\widehat{d}(\bar{s})\ge \frac{\epsilon}{6D}$}
					\State $U\leftarrow U\cup(\bar{s}, \pi)$, and update $\SHP{\pi'}$ for all $\pi'\in\Pi$.
					\State $\mD_{\bar{s}}\leftarrow \mathrm{Sampling}(\Pi_{\exp}, \bar{s}, \pi, N_2)$.
					\State Skip the rest and run next while loop
				\EndIf
			\EndFor
		\EndFor
		\State break the while loop.
		\EndWhile
	\end{algorithmic}
\end{algorithm} 

\par After the \textbf{Identification} process, we will output the set $U$, where we know for every $\pi\in \Pi$ and $s\in \mS^\pi\backslash U$, \eqref{eq:srem} holds. This property, as we will show later, will be the key property that guarantees that the \textbf{Evaluation} Algorithm (\pref{alg:eval}) outputs an $\epsilon$-close estimation to $V^\pi$. The structure of \pref{alg:eval} is similar to \pref{alg:identify}. Suppose we already got the desired set $U$ of state-policy pairs. We collect datasets $\mathcal{D}_0$ and $\mathcal{D}_s$ based on $U$ according to \pref{alg:sample}. For every $\pi\in \Pi$, only datasets $\mD_s$ where $s\in \SHP{\pi}\cap \{0\}$ are useful, and \pref{alg:eval} carries 
an additional processing step (line 1) on datasets $\mathcal{D}_0$ and $\mathcal{D}_s$, i.e. removing all trajectories which passes through the 'problematic' states $\SRem{\pi} = \mS_\pi\backslash U_s$. Meanwhile, for every $s\in \SHP{\pi}\cap\{0\}$, we check whether we remove at least half of the data from $\mD_s$. If so, the estimation based on $\mD_s$ will be inaccurate (in line 8 our algorithm, we directly set the transitions from those states directly to the end state). However, we can also show that these states have very small occupancy from $\pi$ hence the inaccurate estimation will not affect the evaluation of value function very much.

\par For those states in $s\in \SHP{\pi}\cap\{0\}$ and the removal process doesn't delete half of the dataset, we can still get accurate enough estimations. Hence, we adopt the importance sampling (line 5) to 


\begin{algorithm}
	\caption{Evaluate$(\Pi_{\exp}, \mD_0, \mD_s, U, \pi)$}\label{alg:eval}
	\begin{algorithmic}[1] 
	%\State For $s\in U_s\cup\{0\}$, let
	%$$\bar{\mD}_s\leftarrow \left\{\tau:\tau\in\mD_s, \forall s'\in \SRem{\pi}, s'\not\in \tau\right\}.$$
		\For{$s\in(\SHP{\pi})\cup \{0\}, s'\in\SHP{\pi}\cup\{e\}$} 
				\State Calculate $\widehat{P}_{s\to s'}^\pi, \widehat{r}_{s\to s'}^\pi$ according to \eqref{eq:tab};
		\EndFor
		\State $\widehat{V}^\pi\leftarrow \mathrm{DP}(\SHP{\pi}\cup\{0, e\}, \widehat{P}_{s\to s'}^\pi, \widehat{r}_{s\to s'}^\pi)$.
		\State Return $\widehat{V}^\pi$.
	\end{algorithmic}
\end{algorithm}




\subsection{Analysis of the Algorithnm}
\par We have the following theorem
\begin{theorem}\label{thm:core}
	If \pref{ass:core_policy} and \pref{ass:coverage} holds, then \pref{alg:main} will return a $\epsilon$-optimal policy with probability at least $1 - \delta$.
\end{theorem}

\par The proof of this Theorem is divided into two parts. In the first part, we demonstrate that the number of while loop in \pref{alg:identify} is upper bounded (hence the size of $U$ is upper bounded), and also if \pref{alg:identify} terminates, we will have for any $\pi\in \Pi$ and $s\in \SRem{\pi} = \mS_\pi\backslash U_s$, we have
$$d^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{12D}.$$
In the second part, we will show that if the above inequality holds, then \pref{alg:eval} will return an $\epsilon$-close value function with high probability.

\begin{lemma}[Simulation Lemma]\label{lem:sim}
	Suppose $V = \text{DP}(\mS, P, r)$ and $\widehat{V} = \text{DP}(\mS, \widehat{P}, \widehat{r})$, then we have
	$$\left|V - \widehat{V}\right|\le 2\sum_{s\in \mS} d(s)\cdot \left(\sum_{s'\in\mS} \left|P_{s\to s'} - \widehat{P}_{s\to s'}\right| + \left|r_{s\to s'} - \widehat{r}_{s\to s'}\right|\right),$$
	where $d(s)$ is the occupancy measure of $s$ under transition model $P$.
\end{lemma}
\begin{proof}
	
\end{proof}

\begin{lemma}\label{lem:identify}
	If during the while loop in \pref{alg:identify}, line 9 is called, then we have $d^{\pi}(\bar{s})\ge \frac{\epsilon}{12D}$. If the while loop is broken, then for any $\pi\in \Pi$ and $s\in\SRem{\pi}$, we have $d^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{4D}$.
\end{lemma}
\begin{proof}
	First note that every while loop must add at least $(s, \pi)$ where $s\in\mS_\pi$ into $U$. Therefore, $|U|\le D|\Pi|$, and the while loop will iterative at most $D|\Pi|$ times.

	We will prove by induction that at any while loop, if $(s, \pi)\in U$, then we have $d^{\pi}(s)\ge \frac{\epsilon}{12D}$. At the first round the argument obviously holds since $U = \emptyset$.

	\par Suppose at the current while loop, for all $(s, \pi)\in U$, $d^{\pi}(s)\ge \frac{\epsilon}{12D}$, we will prove that if we add a new pair into $U$, it still satisfies this argument. 
	
	\par For some $(s, \pi)\in U$, since $d^{\pi}(s)\ge \frac{\epsilon}{12D}$, according to Hoeffding inequality with probability at least $1 - \delta$, we have
	$$\left|\frac{|\mD_s|}{N_2} - \frac{\epsilon}{12D}\right|\le \sqrt{\frac{2\log(1/\delta)}{N_2}},$$
	which indicates that when $N_2\ge \frac{1152D^2\log(1/\delta)}{\epsilon^2}$, with probability at least $1 - \delta$ we have
	$$|\mD_s|\ge \frac{\epsilon N_2}{24D}.$$
	Therefore, with probability at least $1 - |U_s|\delta\ge 1 - D|\Pi|\delta$, we have for all $s\in U_s$, $|\mD_s|\ge \frac{\epsilon N_2}{24D}$. In the next, we will conditioned on this event.
	
	\par Next, for any trajectory $\tau$, and policy $\pi$, we use $P^{\pi}(\tau)$ to denote the probability of getting $\tau$ from sampling a trajectory from $\pi$. We further denote the probability of getting this $\tau$ in line 2-3 of \pref{alg:sample} to be $\PIS(\tau)$ (and expectation to be $\EE^{\mathrm{IS}}$). Then we have
	$$\PIS(\tau) = \frac{1}{|\Pi_{\exp}|}\sum_{\pi_e\in \Pi_{\exp}} P^{\pi'}(\tau).$$
	We remember
	$$\widehat{P}_{s\to s'} = \frac{|\Pi_{\exp}|}{|\mD_s|}\sum_{\tau\in \mD_s}\frac{\mathbb{1}[\tau[s, s']\sim \pi]}{\sum_{\pi_e\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]}\mathbb{1}[\tau\in \event{s}{s'}{\mS_{\pi}}].$$
	Without loss of generality, we assume $s\in \mS_{h}$ and $s'\in \mS_{h'}$ where $h < h'$. For $s\neq 0$, $\tau[s, s']$ where $\tau\in\mD_s$ can be viewed as $i.i.d.$ sampled from (1) $\pi_e\sim \mathrm{Unif}(\Pi_{\exp})$, (2) sample an $h' - h$ length trajectory starting from $s$ in layer $h$. According to \pref{ass:core_policy}, for any $\tau[s, s'] = (s_h, a_h, s_{h+1}, \cdots, s_{h'})$ such that
	$$\tau[s, s']\sim \pi\quad \text{ and }\quad \tau\in \event{s}{s'}{\mS_{\pi}},$$
	there exists some $\pi_e\in\Pi_{\exp}$ such that $\tau[s, s']\sim \pi_e$, which indicates that $\pi_e(s_i) = a_i = \pi(s_i)$ for every $h\le i\le h'-1$. Hence
	\begin{align*}
		P^{\pi}[\tau[s, s']] & = \prod_{i=h}^{h'-1} P(s_{h+1}|s_h, \pi(s_h)) = \prod_{i=h}^{h'-1} P(s_{h+1}|s_h, \pi_e(s_h)) = P^{\pi_e}[\tau[s, s']]\\
		& = \frac{1}{|\Pi_{\exp}|}\sum_{\pi_e\in \Pi_{\exp}}P^{\pi_e}[\tau[s, s']\sim \pi_e] = \PIS[\tau[s, s']],
	\end{align*}
	which indicates that
	$$\mathbb{E}^{\mathrm{IS}}\left[\frac{\mathbb{1}[\tau[s, s']\sim \pi]\mathbb{1}[\tau\in \event{s}{s'}{\mS_{\pi}}]}{\frac{1}{|\Pi_{\exp}|}\sum_{\pi_e\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]}\right] = \mathbb{E}^{\mathrm{IS}}\left[\frac{P^{\pi}[\tau[s, s']]}{\PIS[\tau[s, s']]}\right] = P_{s\to s'}.$$
	Moreover, \pref{ass:core_policy} indicates that for any $\tau$ such that $\tau[s, s']\sim \pi, \tau\in\event{s}{s'}{\mS_\pi}$, we have $\sum_{\pi_e\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]\ge 1$. Hence 
	$$\frac{\mathbb{1}[\tau[s, s']\sim \pi]\mathbb{1}[\tau\in \event{s}{s'}{\mS_{\pi}}]}{\frac{1}{|\Pi_{\exp}|}\sum_{\pi_e\in \Pi_{\exp}}\mathbb{1}[\tau[s, s']\sim \pi_e]}\in [0, |\Pi_{\exp}|]$$
	always holds.
	Hence according to Hoeffding inequality, for any $s\in\SHP{\pi}$ and $s'\in \mS_\pi\cup\{e\}$, with probability at least $1 - \delta$ we have
	$$\left|\widehat{P}_{s\to s'} - P_{s\to s'}\right|\le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{|\mD_s|}}\le |\Pi_{\exp}|\sqrt{\frac{48D\log(1/\delta)}{\epsilon N_2}}.$$
	Similarly, we can also get for any $s'\in\mS_\pi\cup\{e\}$, 
	$$\left|\widehat{P}_{0\to s'} - P_{0\to s'}\right|\le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{|\mD_0|}} = |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1}}.$$
	
	\par According to \pref{lem:sim}, with probability at least $1 - \log\left(|\Pi|(D+1)^2\delta\right)$, the output $\widehat{d}(\bar{s})$ in line 7 satisfies
	\begin{align*}
		\left|\widehat{d}(\bar{s}) - \bar{d}^{\pi}(\bar{s}, \SRem{\pi})\right| & \le 2\sup_{s\in\SHP{\pi}\cup\{0\}} (D+1)\cdot \sup_{s'\in \mS_\pi\cup\{e\}}|\widehat{P}_{s\to s'} - P_{s\to s'}| \\
		& \le 2(D+1)|\Pi_{\exp}|\left(\sqrt{\frac{48D\log(1/\delta)}{\epsilon N_2}} + \sqrt{\frac{2\log(1/\delta)}{N_1}}\right).
	\end{align*}
	Hence if choosing $N_2\gtrsim \frac{D^5|\Pi_{\exp}|^2\log(|\Pi|D\delta)}{\epsilon^3}$, and $N_1\gtrsim \frac{D^4|\Pi_{\exp}|^2\log(|\Pi|D\delta)}{\epsilon^2}$, we will have in each while loop, $\left|\widehat{d}(\bar{s}) - \bar{d}^{\pi}(\bar{s}, \SRem{\pi})\right|\le \frac{\epsilon}{12D}$ holds for all $\pi$ and $\bar{s}$. This indicates that if we add a new $(s, \pi)$ into $U$, we will have 
	$$\bar{d}^{\pi}(\bar{s}, \SRem{\pi})\ge \frac{\epsilon}{6} - \frac{\epsilon}{12} = \frac{\epsilon}{12}.$$
	Hence noticing that $\bar{d}^{\pi}(\bar{s}, \SRem{\pi})\le d^{\pi}(\bar{s})$, the induction hypothesis is proved for the next round.
	
	\par Additionally, we know that if the while loop is broken, then for every $\pi\in \Pi$ and $\bar{s}\in\SRem{\pi}$, we all have $\widehat{d}(\bar{s})\le \frac{\epsilon}{6}$. Hence we get
	$$\bar{d}^{\pi}(\bar{s}, \SRem{\pi})\le \frac{\epsilon}{4D}.$$
\end{proof}


\begin{lemma}
	The while loop will end in at most $\frac{12DC(\Pi, M)}{\epsilon}$ rounds.
\end{lemma}
\begin{proof}
	According to \pref{lem:identify}, we know that for any $(s, \pi)\in U$, we have
	$$d^{\pi}(s)\ge \frac{\epsilon}{12D}.$$
	Additionally, according to \pref{ass:coverage}, we have that
	$$\sum_{s\in\mS}\sup_{\pi\in \Pi}d^{\pi}(s)\le C(\Pi, \mathcal{M}).$$
	Suppose for any $s\in U_s$, $(\pi, s)\in U$. Noticing that in each while loop, one new $s$ will be added into $U_s$, we get
	$$\frac{\epsilon}{12D}\cdot |U|\le \sum_{s\in U_s} d^{\pi_s}(s)\le \sum_{s\in\mS} \sup_{\pi\in\Pi}d^{\pi}(s)\le C(\Pi, \mathcal{M}),$$
	which indicates that
	$$|U|\le \frac{12DC(\Pi, M)}{\epsilon}.$$
	And the while loop will also end in $\frac{12DC(\Pi, \mathcal{M})}{\epsilon}$ rounds.
\end{proof}


\begin{lemma}
	Fix $\pi\in\Pi$, suppose for any $s\in\SRem{\pi}$ we have
	$$\bar{d}^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{4D},$$
	then the output of $\widehat{V}^\pi$ in \pref{alg:eval} satisfies
	$$\left|\widehat{V}^\pi - V^\pi\right|\le \epsilon$$
\end{lemma}
\begin{proof}
	Additional to the definition of $P_{s\to s'}$ in \eqref{eq:original}, for $s\in\mS_h$ and $s'\in\mS_{h'}$ we define
	$$r_{s\to s'} = \EE_{\tau\sim \pi}\left[R(\tau[s:s'])\mathbb{1}[\tau\in \event{s}{s'}{\mS_\pi}]\big|s_h = s\right].$$
	Then we have the following claim:
	\begin{align*}
		\left|r_{s\to s'} - \widehat{r}_{s\to s'}\right| & \le |\Pi_{\exp}|\sqrt{\frac{48D\log(1/\delta)}{\epsilon N_2}}, \quad \forall s\in\SHP{\pi},\\
		\left|r_{s\to s'} - \widehat{r}_{s\to s'}\right| & \le |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1}}, \quad \forall s = 0,
	\end{align*}
	\par We notice that $\sum_{s\in\mS_\pi} P_{s\to s'} = 1$. Hence we construct the following Markov Reward Process $\bar{M}_{\mathrm{tab}}^\pi$, with state space to be $\{0, e, v\}\cup \SHP{\pi}$:
	\begin{align*}
		\bar{P}_{s\to s'} = P_{s\to s'}, r_{s\to s'} = r_{s\to s'}, \quad \forall s\in \{0\}\cup\SHP{\pi}, s'\in \SHP{\pi}\cup\{e\},\\
		\bar{P}_{s\to o} = 1 - \sum_{s'\in\SHP{\pi}\cup\{e\}} P_{s\to s'} = \sum_{s'\in\SRem{\pi}} P_{s\to s'}, r_{s\to o} = 0,\quad \forall s\in\{0\}\cup\SHP{\pi},\\
		\widehat{P}_{e\to o} = \bar{P}_{o\to o} = 1, \widehat{r}_{e\to o} = r_{o\to o} = 0.
	\end{align*}
	Suppose the value function of $\bar{M}_{\mathrm{tab}}^\pi$ to be $\bar{V}_{\mathrm{tab}}^\pi$. Notice that if we let
	$$\widehat{P}_{s\to o} = \bar{P}_{s\to o}, \widehat{r}_{s\to o} = \bar{r}_{s\to o} = 0,$$
	then $\mathrm{DP}(\SHP{\pi}\cup\{0, e, o\}, \widehat{P}, \widehat{r})$ exactly matches the output of \pref{alg:eval}, since we will have $V(o)\equiv 0$ in \pref{alg:dyna}. Then according to \pref{lem:sim}, we get
	\begin{align*}
		\left|\widehat{V}^{\pi} - \bar{V}_{\mathrm{tab}}^\pi\right| & \le 2(D+2)\sup_{s\in\SHP{\pi}\cup\{0\}, s'\in\SHP{\pi}\cup\{e, o\}}\left(\left|\bar{P}_{s\to s'} - \widehat{P}_{s\to s'}\right| + \left|\bar{r}_{s\to s'} - \widehat{r}_{s\to s'}\right|\right)\\
		& \le 4(D+2)\left(|\Pi_{\exp}|\sqrt{\frac{48D\log(1/\delta)}{\epsilon N_2}}\vee |\Pi_{\exp}|\sqrt{\frac{2\log(1/\delta)}{N_1}}\right)\le \frac{\epsilon}{2}
	\end{align*}
	
	\par Additionally For any $s_{h_1} = 0, s_{h_2}, \cdots, s_{h_{t-1}}, s_{h_t} = e\in\{0, e\}\cup \SHP{\pi}$, 
	\begin{align*}
		&\quad P^{\bar{M}_{\mathrm{tab}}^\pi}(\bar{\tau} = (s_{h_1}, s_{h_2}, \cdots, s_{h_t})) = \prod_{i=1}^{t-1}\bar{P}_{s_{h_i}\to s_{h_{i+1}}} = \prod_{i=1}^{t-1}P_{s_{h_i}\to s_{h_{i+1}}}\\
		& = \prod_{i=1}^{t-1} P^{\pi, M}(\tau:\tau\in \event{s_{h_i}}{s_{h_{i+1}}}{\mS_\pi}|\tau[h_i] =s_{h_i})\\
		& = P^{\pi, M}(\tau: \tau[h_i] = s_{h_i}, \forall 1\le i\le t, \tau[h]\not\in \mS_\pi, \forall h\neq h_1, \cdots, h_t).
	\end{align*}
	Similarly, we can also get
	\begin{align*}
		&\quad \EE^{\bar{M}_{\mathrm{tab}}^\pi}(R[\bar{\tau}]\mathbb{1}[\bar{\tau} = (s_{h_1}, s_{h_2}, \cdots, s_{h_t})])\\
		& = \EE^{\pi, M}(R[\tau]\mathbb{1}[\tau[h_i] = s_{h_i}, \forall 1\le i\le t, \tau[h]\not\in \mS_\pi, \forall h\neq h_1, \cdots, h_t]).
	\end{align*}
	Next we notice that state $e, o$ will never induce any reward. Summing over all possible $s_{h_1}, \cdots, s_{h_t}$, we will get
	$$\bar{V}_{\mathrm{tab}}^\pi = \EE^{\pi, M}(R[\tau]\mathbb{1}[\tau\cap \SRem{\pi} = \emptyset]).$$
	Hence since $\forall s\in\SRem{\pi}, \bar{d}^{\pi}(s, \SRem{\pi})\le \frac{\epsilon}{4D}$, we get
	\begin{align*}
		\left|V^{\pi} - \bar{V}_{\mathrm{tab}}^\pi\right| & = \EE^{\pi, M}(R[\tau]) - \EE^{\pi, M}(R[\tau]\mathbb{1}[\tau\cap \SRem{\pi} = \emptyset])\\
		& = \EE^{\pi, M}(R[\tau]\mathbb{1}[\tau\cap \SRem{\pi} \neq \emptyset])\\
		& = \sum_{s\in\SRem{\pi}}\EE^{\pi, M}(R[\tau]\mathbb{1}[s\in\tau, \tau[0:s]\cap \SRem{\pi} = \emptyset])\\
		& \le \sum_{s\in\SRem{\pi}}\bar{d}^{\pi}(s, \SRem{\pi})\le D\cdot \frac{\epsilon}{4D} = \frac{\epsilon}{4},
	\end{align*}
	which indicates that
	$$\left|\widehat{V}^\pi - V^\pi\right|\le \left|V^{\pi} - \bar{V}_{\mathrm{tab}}^\pi\right| + \left|\widehat{V}^{\pi} - \bar{V}_{\mathrm{tab}}^\pi\right|\le \frac{\epsilon}{4} + \frac{\epsilon}{2} < \epsilon.$$
\end{proof}




\subsection{Upper Bound on the Algorithm}

\begin{theorem} Sample complexity upper bound under Assunmptions~\ref{ass:core_policy} and \ref{ass:coverage}. 
\end{theorem}

\begin{enumerate}
    \item Give the Algorithm. 
    \item Say in words what the algorithm is doing. 
    \item Analysis sketch / Proof sketch 
\end{enumerate}

\paragraph{Discussion on the algorithm / Novelty}
